Gradual Sensitivity Typing

Reasoning about the sensitivity of functions with respect to their inputs has interesting applications in various areas, such as differential privacy. In order to check and enforce sensitivity, several approaches have been developed, notably sensitivity type systems. In these systems, sensitivity can be seen as an effect in the sense of type-and-effects systems as originally proposed by Gifford and Lucassen. Because type-and-effect systems can make certain useful programming patterns tedious or overly conservative, there is value in bringing the benefits of gradual typing to these disciplines in order to ease their adoption. In this work, we motivate, formalize, and prototype gradual sensitivity typing. The language GSoul supports both the unrestricted unknown sensitivity and bounded imprecision in the form of intervals. Gradual sensitivity typing allows programmers to smoothly evolve typed programs without any static sensitivity information towards hardened programs with a mix of static and dynamic sensitivity checking. In particular, we show that gradual sensitivity supports recursive functions for which fully static checking would be overly conservative, seamlessly enabling exact runtime sensitivity checks. GSoul satisfies both the gradual guarantees and sensitivity type soundness, known as metric preservation. We establish that, in general, gradual metric preservation is termination insensitive, and that one can achieve termination-sensitive gradual metric preservation by hardening specifications to bounded imprecision. We implement a prototype that provides an interactive test bed for gradual sensitivity typing. This work opens the door to gradualizing other typing disciplines that rely on function sensitivity such as differential privacy, as well as other quantitative type-based reasoning techniques.

==> sections/extensions.tex <==
%!TEX root = ../main.tex
\section{From \GSoulCore to \lambdaGSens}
\label{sec:extensions}

So far we have only presented the core calculus \GSoulCore (along with its runtime semantics, \GSoulEvCore), which does not account for the full \lambdaGSens language we have implemented and used in the introduction (\S\ref{sec:in-action}).
We now describe \lambdaGSens, the superset of \GSoulCore with products, sums and recursive types.
In \secref{sec:gsoul-type-system} we introduce the syntax, type system and runtime semantics of \lambdaGSens.
% We then present the gradual language \lambdaGSens in \secref{sec:ggsoul-type-system}.
Finally, in \secref{sec:gsoul-metatheory}, we discuss the metatheory of \lambdaGSens along with the challenges and necessary changes for proving sensitivity soundness with these new features, especially in the presence of recursive types.

\reviv{
The addition of recursive types requires some care in the design of certain aspects of the language and its metatheory, such as iso-recursive subtyping and the need for a stronger proof technique for metric preservation.
In particular, we need to introduce a new auxiliary subtyping judgment and step indexing for proving sensitivity soundness for \lambdaGSensEv.
However, it is worth noting that other recursive types definitions such as syntax, typing rules, and reduction rules, can be incorporated without the need to modify existing definitions.
Furthermore, product and sum types can be added in a completely modular manner, albeit not without care, specially when considering the gradual interpretation of metric preservation.
}

\subsection{\lambdaGSens: \GSoulCore with Products, Sums, and Recursive Types}
\label{sec:gsoul-type-system}

\begin{figure}[t]

  \begin{small}
  \begin{align*}
    e ::= {}&
      \dots \mid
      \pair{e}{e} \mid
      \fst e \mid
      \snd e \mid
      \rfold{\gty} e \mid
      \runfold e
      & \syntaxLabel{expressions}\\
      \mid {}&
      \ttunit \mid
      \inl^{\gty} e \mid
      \inr^{\gty} e \mid
      \caseof{e}{x}{e}{x}{e} \\
    %
    \gty ::= {}&
      \dots \mid
      \unit \mid
      \cgty \msum \cgty \mid
      \cgty \madd \cgty \mid
      \recT. \cgty
      & \syntaxLabel{types}\\
    %
    \cgty ::= {}&
      \itype{\gty}{\gsenv} \mid
      \recvar
      & \syntaxLabel{type-and-effects}\\
    %
    u ::= {}&
      \dots \mid \ttunit \mid \pair{v_1}{v_2} \mid \inl^{\gty} v \mid \inr^{\gty} v \mid \rfold{\gty} v
      & \syntaxLabel{simple values}
    %
    % \Ectx ::= {}&
    %   \dots \mid
    %   \pair{\Ectx}{e} \mid
    %   \pair{v}{\Ectx} \mid
    %   \fst \Ectx \mid
    %   \snd \Ectx \mid
    %   \rfold{\gty} \Ectx
    %   & \syntaxLabel{evaluation contexts}\\
    %   \mid {}&
    %   \inl^{\gty} \Ectx \mid
    %   \inr^{\gty} \Ectx \mid
    %   \caseof{\Ectx}{x}{e_1}{y}{e_2}
  \end{align*}
  \textbf{Well-typed expressions} \hfill
  \boxed{\ssttyping{e}{\cgty}}\\
  \begin{mathpar}
    \inferrule*[lab=\Grefr{pair}]{
      \sttyping{e_1}{\cgty[1]} \\
      \sttyping{e_2}{\cgty[2]}
    }{
      \sttyping{\pair{e_1}{e_2}}{\itype{(\cgty[1] \madd \cgty[2])}{\emptysenv}}
    }

    \inferrule*[lab=\Grefr{proj1}]{
      \sttyping{e}{\cgty}
    }{
      \sttyping{\fst e}{\fstt(\cgty)}
    }

    \inferrule*[lab=\Grefr{inl},width=12em]{
      \sttyping{e}{\cgty[1]} \\
      \cgty[2] = \itype{\gty[2]}{\emptysenv} \\
      \typewfs{\cgty[2]}
    }{
      \sttyping{
        \inl^{\gty[2]} e
      }{\itype{(\cgty[1] \msum \cgty[2])}{\emptysenv}}
    }

    \inferrule*[lab=\Grefr{case}]{
      \sttyping{
        e_1
      }{
        \cgty[1]
      }\\
      \sttyping[\tenv, x:\leftt(\cgty[1])]{
        e_2
      }{
        \cgty[2]
      }\\
      \sttyping[\tenv, y:\rightt(\cgty[1])]{
        e_3
      }{
        \cgty[3]
      }
    }{
      \sttyping{
        \caseof{e_1}{x}{e_2}{y}{e_3}
      }{
        \cgty[2] \tjoin \cgty[3] \effOp{\sjoin} \eff(\cgty[1])
      }
    }

    \inferrule*[lab=\Grefr{fold}]{
      \sttyping{e}{\cgtyp}\\
      \cgtyp \subty \unff(\itype{(\recT[\recvar].\cgty)}{\emptysenv})
    }{
      \sttyping{\rfold{\recT[\recvar].\cgty} e}{\itype{(\recT[\recvar].\cgty)}{\emptysenv}}
    }

    \inferrule*[lab=\Grefr{unfold}]{
      \sttyping{e}{\cgty}
    }{
      \sttyping{\runfold e}{\unff(\cgty)}
    }
  \end{mathpar}

  \begin{mathpar}
    \fstt(\itype{(\cgty[1] \madd \cgty[2])}{\gsenv}) = \cgty[1] \effOp{+} \gsenv \and
    \leftt(\itype{(\cgty[1] \msum \cgty[2])}{\gsenv}) = \cgty[1] \effOp{+} \gsenv \and
    \rightt(\itype{(\cgty[1] \msum \cgty[2])}{\gsenv}) = \cgty[2] \effOp{+} \gsenv \and
    \unff(\itype{(\recT[\recvar].\cgty)}{\gsenv}) = \rsubst{\teff{(\recT[\recvar].\cgty)}{\emptysenv}}{\recvar}\cgty \effOp{+} \gsenv \and
    \eff(\itype{\gty}{\gsenv}) = \gsenv
  \end{mathpar}
  \end{small}

  \caption{Syntax and type system of \lambdaGSens (excerpt)}
  \label{fig:gsoul-syntax-and-typing}
\end{figure}

Figure \ref{fig:gsoul-syntax-and-typing} presents the syntax and typing rules for \lambdaGSens, as well as the notions of reduction.
The syntax and rules already presented for \GSoulCore are unchanged and hence omitted.
Rules \Grefr{pair}, \Grefr{inl} are standard and analogous to \Grefr{lam}; constructing a pair or an injection has no sensitivity effect.
Similarly to \Grefr{app}, in rule \Grefr{proj1} we use a partial meta-function, $\fstt$, to compute the \typeclsSing{} of the projection.
In \Grefr{case}, the \typeclsPlur{} of the branches are computed using extended type environments where each newly-bound variable is given a \typeclsSing{} computed using the meta-functions $\leftt$ and $\rightt$, which extract the left and right component of the sum \typeclsSing{}, respectively.
Then, the resulting \typeclsSing{} is computed by joining the \typeclsSing{} of each branch, and also joining the effect of reducing the sum expression, accounting for the case where branches do not use the bound variables.
% The join corresponds to the maximum of the sensitivities for each variable, \ie~$\SG{(\senv[1] + \sens[1]\r) \sjoin (\senv[2] + \sens[2]\r)} = (\senv[1] \sjoin \senv[2]) + \max(\sens[1], \sens[2])\SG{\r}$.

To illustrate why we have to join the effect of $e_1$ in the rule \Grefr{case}, consider the open expression $\caseof{z}{x_1}{0}{x_2}{x_2 + x_2}$, a resource set $\svenv = \SG{\r[1], \r[2]}$, and a type environment $\tenv = z:\teff{(\teff{\rtype}{\infty \r[1]} \msum \teff{\rtype}{\r[1]})}{\r[2]}$, then the type derivation follows as:
%
\begin{mathpar}
  \inferrule*[left=\Grefr{case}]{
    \ssttyping{z}{\teff{(\teff{\rtype}{\infty \r[1]} \msum \teff{\rtype}{\r[1]})}{\r[2]}}\\
    \ssttyping[\tenv, x_1:\teff{\rtype}{\infty \r[1] + \r[2]}]{0}{\itype{\rtype}{\emptysenv}}\\
    \ssttyping[\tenv, x_2:\teff{\rtype}{\r[1] + \r[2]}]{x_2 + x_2}{\teff{\rtype}{2\r[1] + 2\r[2]}}
  }{
    \ssttyping{\caseof{z}{x_1}{0}{x_2}{x_2 + x_2}}{\teff{\rtype}{\emptysenv \sjoin (2\r[1] + 2\r[2]) \sjoin \r[2]}}
  }
\end{mathpar}
%
%
The resulting effect is $\SG{(2\r[1] + 2\r[2])} \sjoin \r[2] = \SG{2\r[1] + 2\r[2]}$.
Also notice that if we now change the expression to be $\caseof{z}{x_1}{0}{x_2}{1}$, where the branches are not using their bound variables, then the resulting effect is $\SG{\r[2]}$, the effect of reducing $z$ to a value.

Rule \Grefr{fold} allows for subtyping in its body, and rule \Grefr{unfold} relies on the meta-function $\unff$ which performs a substitution for the recursive variable and integrates the latent effect of the inner expression.
Recursive type substitution $\rsubst{\cdot}{\cdot}\cdot$ replaces a \typeclsSing{} for a recursive variable.
Notice that in the definition of $\unff$, the substitution has an empty effect.
This ensures that the effect of reducing the expression to a fold value is only accounted for once, and not at each unfolding.

\paragraph{Subtyping and Recursive Types.}
A last aspect of \lambdaGSens that we have to take care of is subtyping in the presence of recursive types.
% In both \SoulCore and \lambdaSens, subtyping is derived directly from the notion of ordering of sensitivities and there is no top or bottom type.
% A sensitivity effect is a sub-effect of another if, for each sensitive variable, all sensitivities are no greater than the other.
% Designing sound subtyping rules in the presence of recursive types is subtle.
For this, we adopt the \textit{weakly positive subtyping} approach of \cite{zhouAl:toplas2022}:\footnote{
  We could also have used the standard Amber rules~\cite{cardelli:springer1986}, although as argued by \citet{zhouAl:toplas2022}, the metatheory of iso-recursive Amber rules is challenging;
  their approach is equivalent while enjoying a simpler metatheory.
}
\begin{small}
  \begin{mathpar}
    \inferrule*[lab=\Grefr{sub-rec}]{
      \cgty[1] \subty \cgty[2] \\
      \recvar \wpr[+] \cgty[1] \subty \cgty[2]
    }{
      \recT . \cgty[1] \subty
      \recT . \cgty[2]
    }

    \inferrule*[lab=\Grefr{sub-rec-refl}]{
      \cgty[1] \sim \cgty[2]
    }{
      \recT . \cgty[1] \subty
      \recT . \cgty[2]
    }
  \end{mathpar}
\end{small}
This approach relies on the polarized judgment $\recvar \wpr \cgty[1] \ccsub \cgty[2]$, which checks whether $\recvar$ is used positively or negatively---indicated by the $m$ polarity---in \typeclsPlur{} $\cgty[1]$ and $\cgty[2]$; we write $\negmode{m}$ for flipping the polarity $m$.
Rule \Grefr{sub-rec} allows for subtyping in the bodies of the recursive types under the condition that $\recvar$ only appears in positive positions.
Recursive variables can still appear in negative positions but only for plausibly equal types, described using $\sim$, by rule \Grefr{sub-rec-refl}.\footnote{
  Plausible equality, written $\cgty[1] \sim \cgty[2]$, also known as consistency, is equivalent to $\cgty[1] \ccsub \cgty[2] \land \cgty[2] \ccsub \cgty[1]$.
}
To ensure that subtyping remains deterministic, rule \Grefr{sub-rec-refl} is only used when $\recvar \wpr[+] \cgty[1] \subty \cgty[2]$ is false, otherwise \Grefr{sub-rec} is used.
The definition of the weakly positive restriction can be found in the supplementary material.

\begin{figure}[t]
  \begin{small}
  \textbf{Notions of reduction} \hfill
  \boxed{t \longrightarrow t}\\
  \begin{align*}
    % FIRST
    %
    \IGrefr{r-fst} & &
    \fst (\ev \pair{v_1}{v_2} \ascr{\cgty})
    & \longrightarrow
    \ifirst(\ev) v_1 \ascr{\fstt(\cgty)}\\
    %
    % UNFOLD
    %
    \IGrefr{r-unfold} & &
    \runfold (\ev (\rfold{\cgtyp} v) \ascr{\cgty}) &
    \longrightarrow
    \iunf(\ev) v \ascr{\unff(\cgty)}\\
    %
    % CASE-1
    %
    \IGrefr{r-case-1} & &
    \begin{array}{l}
      \caseKW (\ev[1] \inl^{\gtyp[12]} (\ev[11] u \ascr{\cgtyp[11]}) \ascr{\cgty[1]})\\
      \quad \ofCases{x}{t_2^{\cgty[2]}}{y}{t_3^{\cgty[3]}}
    \end{array}
    &\longrightarrow
    \begin{cases}
      \ev[2]
        (\substv{\evp[11] u \ascr{\leftt(\cgty[1])}}{x}{t_2})
      \ascr{\cgty[2] \tjoin \cgty[3] \effOp{\sjoin} \eff(\cgty[1])}\\
      \error \hspace{1.7cm} \text{\color{black} if not defined}\\
    \end{cases}\\
    \where & &
    \multicolumn{2}{c}{$
      \evp[11] = \ev[11] \transsub \ileft(\ev[1]),\quad
      \ev[2] = \Isub(\cgty[2], \cgty[2] \tjoin \cgty[3]) \effOp{\sjoin}^{\SG{2}} \eff^2(\ev[1])
    $}
  \end{align*}
  \end{small}

  \caption{Reduction rules for \lambdaGSensEv (excerpt)}
  \label{fig:gsoul-reduction}
\end{figure}

\paragraph{Dynamic semantics}
The reduction rules for products, sums, and recursive types are presented in Figure~\ref{fig:gsoul-reduction}.
Evaluation contexts and values are extended with the corresponding constructs, following call-by-value semantics as before.
For rules \IGrefr{r-fst} and \IGrefr{r-snd}, we use inversion functions $\ifirst$ and $\isecond$ analogous to $\icod$.
Then, if evidence $\ev$ justifies $\ev \evjust \cgty[1] \ccsub \cgty[2]$, then $\ifirst(\ev) \evjust \fstt(\cgty[1]) \ccsub \sndd(\cgty[2])$, assuming the types involved are products.
% Although the derivation process is analogous to \IGrefr{r-app}, rule \IGrefr{r-case-1} is more complex.
For rule \IGrefr{r-case-1}, evidence $\evp[11]$, for the \reviv{substituted} value, is computed using the inversion function $\ileft$ (instead of $\idom$ in \IGrefr{r-app}).
Since the body terms have no explicit evidences, in order to produce an evidence $\ev[2]$ for the context term we use the interior operator.
For $\ev[2]$, to fully reflect the type operations made in the ascription, we must join the information in the sensitivity environment parts of $\ev[1]$.
This is done by using the functions $\eff^2$ and $\effOp{\sjoin}^{\SG{2}}$, the lifted versions of $\eff$ and $\effOp{\sjoin}$ for operating on evidences, respectively.
Rule \IGrefr{r-case-2}, corresponding to the $\inr$ case, is left out as its definition is analogous to \IGrefr{r-case-1}.
Finally, the reduction rule \IGrefr{r-unfold} is standard, with the subtlety of the use of inversion operator $\iunf$ for justifying the resulting ascription.

\begin{revb}
\paragraph{Handling recursive functions}
\label{subsec:reducing-recursive-calls}
Let us return to the recursive function example of \secref{sec:in-action}.
First, we introduce rules for typechecking and reducing fixpoints; as in \Fuzz, we can encode fixpoints via the Y-combinator, but in order to simplify the presentation, we here introduce a fixpoint primitive:

\begin{small}
\begin{mathpar}
  \inferrule*[left=\IGrefr{fix}]{
    \ittyping{t}{\cgty}
  }{
    \ittyping{\rfix (f: \cgty).t}{\cgty}
  }

  \inferrule*[lab=\IGrefr{r-fix}]{}{
    \ev (\rfix (f: \cgty).t) \ascr{\cgtyp}
    \longrightarrow
    \ev (\rsubst{\Isub(\cgty, \cgty) (\rfix (f: \cgty).t) \ascr{\cgty}}{f}t) \ascr{\cgtyp}
  }
\end{mathpar}
\end{small}

\begin{reviiib}
\reviv{
  Rules \IGrefr{fix} and \IGrefr{r-fix} are standard, modulo the treatment of evidence.
  In \IGrefr{r-fix}, we use the interior operator to justify the ascription of the substituted term, which in this case is trivial: the ascription type-and-effect is the same as the original, thus the interior operator never fails.
  Finally, since the body of the fixpoint has the same type-and-effect as the fixpoint itself, the original evidence $\ev$ can be used to justify the ascription of the result.
}

We can now define the recursive function $\mathsf{scale}$ of \typeclsSing{} $\polyST[\r]. \Nat \rightarrow \teff{\rtype}{\r} \rightarrow \teff{\rtype}{?\r}$:
\footnote{$\Nat$ is encoded as $\itype{\recT. (\itype{(\itype{\unit}{\emptysenv} \msum \recvar)}{\emptysenv})}{\emptysenv}$; hereafter, we use specific natural numbers instead of their encoding.}
\vspace{-0.1em}
\begin{small}
  \begin{align*}
    \polyS[\r]. \rfix \mathit{scale}. (
    \lambda (n: \Nat, v: \teff{\rtype}{\r}).
    \caseof{
      (\runfold n)
    }{\_}{
      0
    }{\mathit{m}}{
      v + \mathit{scale} \app \mathit{m} \app v
    }
  )
  \end{align*}
\end{small}
Let $n = \ev[n] 2 \ascr{\teff{\Nat}{\emptysenv}}$ and $v = \ev[v] 3 \ascr{\teff{\rtype}{\r[1]}}$, where $\ev[n] = \evi{\emptysenv, \emptysenv}$ and $\ev[v] = \evi{\emptysenv, \r[1]}$ (omitting \tyclsPlur{} in evidences to improve readability).
Then if we reduce the expression $\mathsf{scale}\appS{\SG{\r[1]}} \app n \app v$, after several reduction steps we can observe that the recursive function unfolds as many times as necessary, and so each occurrence of $v$ will simply contribute its sensitivity effect to the final result depending on the remaining operations (in this case, sums):
\vspace{-0.5em}

\begin{small}
\begin{align*}
  \mathsf{scale} \appS{\r[1]} \app n \app v
  & \mapsto^{*}
    \ev[2](
      \ev[v] 3 \ascr{\r[1]}
      + \ev[1](
        \ev[v] 3 \ascr{\r[1]}
        + \ev[0] 0 \ascr{\unknown\r[1]}
      ) \ascr{\unknown\r[1]}
    ) \ascr{\unknown\r[1]}
  % & \mapsto
  %   \ev[2](
  %     \ev[v] 3 \ascr{\r[1]}
  %     + \ev[1](
  %       \evi{\emptysenv, \SG{[1,\infty]}\r[1]} 3 \ascr{\unknown\r[1]}
  %     ) \ascr{\unknown\r[1]}
  %   ) \ascr{\unknown\r[1]}\\
  % & \mapsto
  %   \ev[2](
  %     \ev[v] 3 \ascr{\r[1]}
  %     + \evi{\emptysenv, \SG{[1,\infty]}\r[1]} 3 \ascr{\unknown\r[1]}
  %   ) \ascr{\unknown\r[1]}\\
  % & \mapsto
  %   \ev[2](
  %     \evi{\emptysenv, \SG{[2,\infty]}\r[1]} 6 \ascr{\unknown\r[1]}
  %   ) \ascr{\unknown\r[1]}\\
   \mapsto^{*} \evi{\emptysenv, \SG{[2,\infty]}\r[1]} 6 \ascr{\unknown\r[1]}
\end{align*}
\end{small}
where evidences
  $\ev[2] = \evi{\SG{[1,\infty]}\r[1], \SG{[1,\infty]\r[1]}}$,
  $\ev[1] = \evi{\SG{[1,\infty]}\r[1], \SG{[1,\infty]\r[1]}}$
  and $\ev[0] = \evi{\emptysenv, \SG{?\r[1]}}$
  are the results of each unfolding of the fixpoint.

The important insights of this example come from analyzing the final evidence $\evi{\emptysenv, \SG{[2,\infty]}\r[1]}$.
First, during reduction we have learned that resource $\SG{\r[1]}$ was used at least twice.
Second, notice how the sensitivity of $\SG{\r[1]}$ matches exactly  the value of $n$, namely $2$.
More importantly, this generalizes to any value of $n$: the resulting evidence will always be of the form $\evi{\emptysenv, \SG{[\Gbox{\SG{n}},\infty]}\r[1]}$, \ie~a result that is known to be at least $n$-sensitive in resource $\r[1]$.
And finally, this resulting evidence means that we can use the result in other contexts, without having to consider the result as $\infty$-sensitive in the resources it uses.
In particular, for this example, we can successfully pass the result to a function that requires its argument to be at most $2$-sensitive in $\SG{v}$; but passing it to a function that requires a $1$-sensitive argument would produce a runtime error.
\end{reviiib}
\end{revb}


% \begin{figure}[!t]

%   \begin{small}
%   % \begin{mathpar}
%   %   m ::= + \mid - \and
%   %   \negmode{+} = - \and
%   %   \negmode{-} = +\\
%   % \end{mathpar}

%   % \textbf{Weakly positive restriction} \hfill
%   % \boxed{\recvar \wpr \sty[1] \subty \sty[2]}\\
%   % \begin{mathpar}
%   %   \inferrule*[lab=\Trefr{wpr-arrow}]{
%   %     \recvar \wpr[\negmode{m}] \cty[21] \subty \cty[11] \\
%   %     \recvar \wpr \cty[12] \subty \cty[22]
%   %   }{
%   %     \recvar \wpr
%   %     \cty[11] \rightarrow \cty[12] \subty
%   %     \cty[21] \rightarrow \cty[22]
%   %   }

%   %   \inferrule*[lab=\Trefr{wpr-rec-eq}]{
%   %     \recvar \notin \freevars{\cty}
%   %   }{
%   %     \recvar \wpr
%   %     \recT[\recvarp] . \cty \subty
%   %     \recT[\recvarp] . \cty
%   %   }

%   %   \inferrule*[lab=\Trefr{wpr-rec-neq},width=12em]{
%   %     \recvar \neq \recvarp\\
%   %     \recvar \wpr \cty[1] \subty \cty[2] \\
%   %     \recvarp \wpr[+] \cty[1] \subty \cty[2]
%   %   }{
%   %     \recvar \wpr \recT[\recvarp] . \cty[1] \subty
%   %     \recT[\recvarp] . \cty[2]
%   %   }
%   % \end{mathpar}

%   \textbf{Subtyping} \hfill
%   \boxed{\sty \subty \sty}\\
%   \begin{mathpar}
%     \inferrule*[lab=\Trefr{sub-rec}]{
%       \cty[1] \subty \cty[2] \\
%       \recvar \wpr[+] \cty[1] \subty \cty[2]
%     }{
%       \recT . \cty[1] \subty
%       \recT . \cty[2]
%     }

%     \inferrule*[lab=\Trefr{sub-rec-refl}]{ }{
%       \recT . \cty \subty
%       \recT . \cty
%     }
%   \end{mathpar}
%   \end{small}

%   \caption{Recursive subtyping (excerpt)}
%   \label{fig:subtyping-recursive}
% \end{figure}

\subsection{Metatheory of \lambdaGSens}
\label{sec:gsoul-metatheory}

\begin{figure}[!t]

  \begin{small}
  \begin{align*}
    % Related numbers
    % (v_1, v_2) \in \glrV{\itype{\rtype}{\gsenv}} \iff
    % & (v_1, v_2) \in \glrAtom{\itype{\rtype}{\gsenv}} \land \\
    % & \neg \big( \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \lvert u_1 - u_2 \rvert \big) \\
    % & \text{\textcolor{black}{where}}~ v_i = \evi{\itype{\rtype}{\emptysenv}, \itype{\rtype}{\gsenvp[i]}}\, u_i \ascr{\itype{\rtype}{\gsenv}}\\
    %
    % Related units
    (v_1, v_2) \in \glrV{\itype{\unit}{\gsenv}} \iff
    & (v_1, v_2) \in \glrAtom{\itype{\unit}{\gsenv}}\\
    & \text{\textcolor{black}{where}}~ v_i = \ev[i] \ttunit \ascr{\itype{\unit}{\gsenv}}\\
    %
    % Related functions
    (v_1, v_2) \in \glrV{\itype{(\cgty[1] \rightarrow \cgty[2])}{\gsenv}} \iff
    & (v_1, v_2) \in \glrAtom{\itype{(\cgty[1] \rightarrow \cgty[2])}{\gsenv}} \land \\
    & \big( \forall j \leq k, \svp[1], \svp[2], (v_1', v_2') \in \glrV{\cgty[1]}[j-1].\\
    & ({\sv[1] \app \svp[1]}, {\sv[2] \app \svp[2]}) \in \glrT{\cgty[2] \effOp{+} \gsenv}[j] \big)\\
    %
    % Related type abstractions
    (v_1, v_2) \in \glrV{\itype{(\polyS[\r].\cgty)}{\gsenv}} \iff
    & (v_1, v_2) \in \glrAtom{\itype{(\polyS[\r].\cgty)}{\gsenv}} \land \big(\forall j \leq k, \gsenvpp. \\
    & ({\sv[1] \appS{\gsenvpp}}, {\sv[2] \appS{\gsenvpp}}) \in \glrT{\Xisubst{\cgty}[\r]{\gsenvpp} \effOp{+} \gsenv}[j] \big)\\
    %
    % Related products
    (v_1, v_2) \in \glrV{\itype{(\cgty[1] \madd \cgty[2])}{\gsenv}} \iff
    & (v_1, v_2) \in \glrAtom{\itype{(\cgty[1] \madd \cgty[2])}{\gsenv}} \land \\
    & ({\useFst(v_1)}, {\useFst(v_2)}) \in \glrT{\cgty[1] \effOp{+} \gsenv}[k] \land \\
    & ({\useSnd(v_1)}, {\useSnd(v_2)}) \in \glrT{\cgty[2] \effOp{+} \gsenv}[k]\\
    %
    % Related sums
    (v_1, v_2) \in \glrV{\itype{(\cgty[1] \msum \cgty[2])}{\gsenv}} \iff
    & (v_1, v_2) \in \glrAtom{\itype{(\cgty[1] \msum \cgty[2])}{\gsenv}} \land \\
    & \big( \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \infty
    \\
    & \implies
      ({\useL(\sv[1])}, {\useL(\sv[2])}) \in \glrT{\cgty[1] \effOp{+} \gsenv}[k] \lor \\
    & \phantom{\implies (} ({\useR(\sv[1])}, {\useR(\sv[2])}) \in \glrT{\cgty[2] \effOp{+} \gsenv}[k]
      \big)
    \\
    & \text{\textcolor{black}{where}}~ v_i = \evi{\itype{\gty[i1]}{\emptysenv}, \itype{\gty[i2]}{\gsenvp[i]}}\, u_i \ascr{\itype{(\cgty[1] \msum \cgty[2])}{\gsenv}}\\
    %
    % Related folds
    (v_1, v_2) \in \glrV{\itype{(\mutpe{\cgty})}{\gsenv}} \iff
    & (v_1, v_2) \in \glrAtom{\itype{(\mutpe{\cgty})}{\gsenv}} \land \big(\forall j \leq k,\\
    &  ({\unfold{\sv[1]}}, {\unfold{\sv[2]}}) \in \glrT{\substv{\itype{(\mutpe{\cgty})}{\emptysenv}}{\alpha}{\cgty} \effOp{+} \gsenv}[j] \big)\\
    % Related computations
    ({t_1}, {t_2}) \in \glrT{\cgty} \iff &
    \forall j < k.
    (\creds[]{t_1}{\sv[1]}[j] \land
    \creds[]{t_2}{\sv[2]}) \implies
    (v_1, v_2) \in \glrV{\cgty}[k-j]
    %
    % Related environments
    % (\venv[1], \venv[2]) \in \glrG{\tenv} \iff
    % & \dom(\venv[1]) = \dom(\venv[2]) = \dom(\Gamma) ~\land\\
    % & \forall x \in \dom(\Gamma). (\venv[1](x),\venv[2](x)) \in \glrV{\Gamma(x)}
  \end{align*}

  \begin{mathpar}
    \useL(\ev (\inl^{\cgty[12]} v) \ascr{\cgty}) = \ileft(\ev) v \ascr{\leftt(\cgty)} \and
    \useR(\ev (\inr^{\cgty[12]} v) \ascr{\cgty}) = \iright(\ev) v \ascr{\rightt(\cgty)} \and
    \useFst(\ev \pair{v_1}{v_2} \ascr{\cgty}) = \ifirst(\ev) v_1 \ascr{\fstt(\cgty)} \and
    \useSnd(\ev \pair{v_1}{v_2} \ascr{\cgty}) = \isecond(\ev) v_2 \ascr{\sndd(\cgty)}
  \end{mathpar}
  \end{small}

  \caption{Logical relations for gradual sensitivity soundness of \lambdaGSensEv (excerpt)}
  \label{fig:gradual-logical-relation}
\end{figure}

\lambdaGSens satisfies all the properties of the core gradual language.
More notably, it also satisfies both termination-insensitive and -sensitive gradual metric preservation, as well as their respective corollaries.
One important difference between \GSoulCore and \lambdaGSens is that the latter supports general recursion.
This has a direct impact on the proof of sensitivity soundness for \lambdaGSens, because the logical relation presented in \secref{sec:gradual-metric-preservation} is not well-founded in the presence of recursion.
To overcome this, we modify the definition of the logical relations to use \emph{step indexing}~\cite{ahmed:esop2006,appelMcAllester:toplas2001}.
We now discuss the step-indexed logical relation, presented in Figure~\ref{fig:gradual-logical-relation}.

\paragraph{(A) Related numbers, booleans and unit}
Numbers and booleans are related as defined in Figure~\ref{fig:basic-gradual-logical-relation}, independently of the step index.
Two values of the unit type are necessarily equal, and hence related for any step index.

\paragraph{(B) Related functions and resource abstractions}
The definitions remain similar to the ones in \secref{sec:gradual-metric-preservation}, but now they are indexed by a step index $k$.
Two functions are related at \typeclsSing $\itype{(\cgty[1] \to \cgty[2])}{\gsenv}$ {\em for $k$ steps} if, for any $j \leq k$, their applications to two related arguments for $j-1$ steps yield related computations for $j$ steps.
Similarly, two resource abstractions are related for $k$ steps if, for any $j \leq k$, their applications to any sensitivity environment yield related computations for $j$ steps.
Notice that for these cases, although the same step index can used in the recursive definition (when $j = k$), the interpretations are well-founded because in each case a reduction step is always performed, lowering the index by one.

\paragraph{(C) Related pairs and injections}
Two pairs are related simply if each of their components are related.
Any two injections are related for any step index if the predicted (worst-case) output distance $\denv \cdot (\gsenvp[1] \sjoin \gsenvp[2])$ is infinity.
If it is possible that the predicted output distance is less than infinity, then the injections must be either both left injections or right injections.
Furthermore, the underlying values must be related.
Also, and as in the case of booleans, in order to account for the worst case scenario, we need to take the best case on the hypothesis side of the implication as the predicate is in a contravariant position. Therefore, the consistently-less-than operator $\cclt$ is used directly, without the need for double negation.
Finally, the partial meta-functions $\useL$, $\useR$, $\useFst$, and $\useSnd$ are defined to extract the underlying values of the injections and pairs.

\paragraph{(D) Related folds}
Analogous to functions, two folds are related for $k$ steps if, for any $j \leq k$, their unfolding yield related computations at the expected \typeclsSing---as computed by $\unff$ in \Grefr{unfold}---for $j$ steps.

\paragraph{(E) Related computations}
A pair of closed terms are related for $k$ steps whenever the first term reduces to a value in $j$ steps (where $j < k$) and the second reduces to a value in any number of steps, and those two values are related at that type for $k-j$ steps.
Notice that this definition, similar to the first logical relation presented in \secref{sec:gradual-metric-preservation}, is termination-insensitive.
Later in this section, we will revisit the topic of termination-sensitive soundness for \lambdaGSensEv.

We can now state the fundamental property of the logical relation for \lambdaGSensEv, as well as gradual metric preservation for \lambdaGSens.

\begin{restatable}[Fundamental Property for \lambdaGSensEv]{theorem}{gradualMetricPreservation}
  \label{prop:gsoul-gradual-metric-preservation}
  \reviv{Let $t$ be a \lambdaGSensEv term.}
  If $\ittyping{t}{\cgty}$ and $t \vdash \tenv$,
  then $\forall \denv, k\geq0, \venv[1], \venv[2]$ such that $\tenv \vdash \denv$ and $(\venv[1], \venv[2]) \in \glrG{\tenv}$,
  we have $(\venv[1](t), \venv[2](t)) \in \glrT{\cgty}$.
\end{restatable}

\begin{restatable}[Gradual metric preservation for \reviv{\lambdaGSens} base types]{corollary}{gradualMetricPreservationBaseTypes}
  \label{prop:gsoul-gradual-metric-preservation-base-types}
  \reviv{Let $f$ be a \lambdaGSens function.}
  If $f$ has type $\teff{(\teff{\rtype}{\r} -> \teff{\rtype}{\gsens \r})}{\emptysenv}$, for some gradual sensitivity $\gsens$, then
  for any real numbers $c_1, c_2, c$ such that $\abs{c_1 - c_2} \leq c$,
  if $\reval{f \app c_1}{v_1}$, and
  $\reval{f \app c_2}{v_2}$, then
  $\abs{\uval{v_1} - \uval{v_2}} \leq c \cdot\pi_2(\gsens)$.
\end{restatable}

% \begin{figure}

%   \begin{small}
%     \begin{align*}
%       % Related atoms
%       (v_1, v_2) \in \tsglrAtom{\cgty} \iff
%       & \ittyping{\sv[1]}{\cgty} \land \ittyping{\sv[2]}{\cgty} \land {\getev(v_1) = \getev(v_2)}\\
%       % Related terms
%       (t_1, t_2) \in \tsglrT{\cgty}[k] \iff
%       &
%         \forall j < k.
%         \creds[]{t_1}{v_1}[j]
%         \implies ({\exists v_2 . \creds[]{t_2}{v_2}[*]} \land (v_1, v_2) \in \tsglrV{\cgty}[k - j])
%     \end{align*}
%   \end{small}

%   \caption{Termination-sensitive gradual metric preservation}
%   \label{fig:ts-gradual-logical-relation-step-index}
% \end{figure}

\paragraph{Revisiting termination-sensitive gradual metric preservation}
Recursive types not only introduce the need for step indexing in the logical relation, but also make program divergence a possibility.
This requires us to revisit what termination-sensitive gradual metric preservation means.
The attentive reader may have noticed that in \secref{sec:tsmp} we mostly discuss about \emph{different termination behavior across runs} and not specifically about error behavior.
Indeed, the changes made in that section are sufficient to also capture divergence as a possible source of different runs not having uniform termination behavior.
We thus refer to non-termination as both divergence and failure.

For stating termination-sensitive gradual metric preservation for \lambdaGSens we follow the same approach as in \secref{sec:tsmp}: first, we use a second logical relation that requires evidences of related values to be identical; and second, we disallow possibly-infinite distances in the fundamental property.
Again, the definitions for related values remain unchanged with respect to Figure~\ref{fig:gradual-logical-relation}, but the logical relations for terms have to be (trivially) updated to use step indexes.
We can now prove termination-sensitive gradual metric preservation for \lambdaGSens.

\begin{restatable}[(Termination-sensitive) Fundamental Property for \lambdaGSensEv]{theorem}{tsgradualMetricPreservation}
  \label{prop:gsoul-ts-gradual-metric-preservation}
  \reviv{
    Let $t$ be a \lambdaGSensEv term.
  }
  If $\ittyping{t}{\itype{\gty}{\gsenv}}$, $t \vdash \tenv$ and $\neg (\infty \ccleq \denv \cdot \gsenv)$,
  then $\forall \denv, k\geq0, \venv[1], \venv[2]$ such that $\tenv \vdash \denv$ and $(\venv[1], \venv[2]) \in \tsglrG{\tenv}$,
  we have $(\venv[1](t), \venv[2](t)) \in \tsglrT{\itype{\gty}{\gsenv}}$.
\end{restatable}

\begin{restatable}[Termination-sensitive gradual metric preservation for base types]{corollary}{gradualMetricPreservationBaseTypesTS}
  \label{prop:gsoul-gradual-metric-preservation-base-types-TS}
  \reviv{Let $f$ be a \lambdaGSens function.}
  If $f$ has type $\teff{(\teff{\rtype}{\r} -> \teff{\rtype}{\gsens \r})}{\emptysenv}$,
  for some gradual sensitivity $\gsens$, then
  for any real numbers $c_1, c_2, c$ such that $\abs{c_1 - c_2} \leq c$ and $c \cdot \pi_2(\gsens) < \infty$,
  if $\reval{f \app c_1}{v_1}$ then
  $\reval{f \app c_2}{v_2}$ and
  $\abs{\uval{v_1} - \uval{v_2}} \leq c\cdot\pi_2(\gsens)$.
\end{restatable}

All the proofs for \GSoulCore and \GSoulEvCore are subsumed by the proofs for \lambdaGSens and \lambdaGSensEv, which can be found in the supplementary material.


==> sections/gmp.tex <==

\section{A Gradual Metatheory for Sensitivity}
\label{sec:a-gradual-metatheory}

% \begin{small}
% \begin{align*}
%   \tenv &= b : \btype, x : \rtype \\
%   e &= \mathsf{if} \ b \ \mathsf{then} \ (x + x) \ \mathsf{else} \ (x + x + x) \\
%   \syntypingMP[\tenv&]{e}{\itype{\rtype}{b + 3x}} \\
%   \venv &= \set{b \mapsto \mathsf{true}, x \mapsto 4@x} \\
%   \reval{e&}{8@(b + 2x)}
% \end{align*}
% \end{small}

The cornerstone of this work are {\em gradual sensitivities}, which represent {\em imprecise} sensitivity information that is optimistically handled by the type system.
Recall from \S\ref{sec:in-action} that we support both unbounded imprecision via the fully-unknown sensitivity $\unknown$ and bounded imprecision via sensitivity intervals such as $\sensint{1, 10}$.
A gradual sensitivity $\gsens$ is defined as a valid interval of two static sensitivities, capturing the plausibility of a sensitivity being any number within the range.
Note that the unknown sensitivity $\unknown$ is sugar for the interval $\sensint{0, \infty}$, and a \textit{fully precise} sensitivity $\sens$ is sugar for the interval $\sensint{\sens,\sens}$:%
% For example, the gradual sensitivities $\sensint{0, \infty}$ and $\sensint{3, 3}$ can also be written as $\unknown$ and $\sensval{3}$, respectively.
%Formally, we define the syntax of gradual sensitivities as follows:
\footnote{
  By extension, types, expressions and type environments may be gradual.
  Nevertheless, we use the same meta-variables as in the syntax presented earlier.
}

\begin{small}
\begin{align*}
  \gsens &::= \sensint{\sens[1], \sens[2]} &
  \text{with:} \quad
  \unknown \triangleq \sensint{0, \infty}, \quad \sens \triangleq \sensint{\sens, \sens} \\
  \gsenv &::= \gsens x + \dots + \gsens x
\end{align*}
\end{small}

\begin{comment}
\da{introduce nicely}\mt{why do we need precision at this point?}
Precision in the context of gradual sensitivities corresponds to interval inclusion.
Formally, $\sensint{\sens[1], \sens[2]}$ is more precise than $\sensint{\sens[3], \sens[4]}$, written $\sensint{\sens[1], \sens[2]} \gprec \sensint{\sens[3], \sens[4]}$, if and only if $\sens[1] \geq \sens[3]$ and $\sens[2] \leq \sens[4]$.
Precision for gradual sensitivity effects, \tyclsPlur and \typeclsPlur is naturally defined from gradual sensitivities precision, \eg~${\sensint{2, 8}x + \sensint{2,\infty}y} \gprec {\sensint{0, 10}x + \unknown y}$ because $\sensint{2, 8} \gprec \sensint{0, 10}$ and $\sensint{2, \infty} \gprec \sensint{0, \infty}$.
\end{comment}

Optimism for gradual sensitivities arises from relaxing the order of sensitivities, which yields an optimistic order for gradual sensitivities, denoted by $\ccleq$.
Intuitively, a gradual sensitivity $\gsens[1]$ is optimistically less or equal to another, $\gsens[2]$, if there \emph{exists} a sensitivity within $\gsens[1]$ that is less or equal to another one within $\gsens[2]$.
This is easily checkable by comparing the lower bound of $\gsens[1]$ with the upper bound of $\gsens[2]$, which corresponds to the best-case scenario.
Formally, we define:

\begin{definition}[Consistent Sensitivity Order]
  \label{def:consistent-sens-subtyping}
  $\sensint{\sens[1], \sens[2]} \ccleq \sensint{\sens[3], \sens[4]}$ if and only if $\sens[1] \leq \sens[4]$.
\end{definition}

Just like with static sensitivities, this consistent sensitivity order induces an (optimistic) order for gradual sensitivities environments, types and sensitivity types.
We write $\ccleq$ for sensitivity environments, and $\ccsub$ for types and sensitivity types, calling the latter \emph{consistent subtyping}.

The imprecision of gradual sensitivities allow a gradual language to be optimistic during static typechecking, and to detect, via runtime checks, if an optimistic static assumption turns out to be violated during execution, thereby raising an error.
Therefore, the runtime semantics of a language with gradual sensitivities must perform both {\em tracking} and {\em checking} of sensitivity information.

For the rest of the section, we equip the calculus with an abstract operational semantics in which expressions reduce to tagged values, written $\reval{e}{\tagged{u}[\tg]}$.
Furthermore, an expression may also reduce to an error, written $\reval{e}{\error}$, as one would expect from a gradual language.
Tags, for now abstract in their representation, carry information about the sensitivity of the value they tag.
As so, we use the meta-function $\getS$ to extract the {\em monitored} sensitivity environment from a tag, which corresponds to the sensitivity of the expression that produced the value.
For instance, giving $x$ a proper value, we could have $\reval{x + x}{\tagged{4}[\tg]}$ where $\getS(\tg) = 2x$, noting that $2x$ is not the sensitivity of the constant literal $4$ but rather the sensitivity of the computation that produced it.


\begin{comment}

  % In order to continue with the development of a metatheory for gradual sensitivities, we present the operational semantics for a variation of the lambda calculus used in the previous section,
  % Importantly, the tracked information may be checked against other tags, which may contain contradictory information.
  % We take inspiration on security typing systems\da{cite}\mt{zdancewic thesis?}\mt{maybe about language that reason about information flow}, which are designed around the notion of labeled values, whose security information flows through the program, \ie~tainting the expressions they interact with.
  % Nevertheless, our approach considers not only tainting but also runtime checks that may fail.
  % The syntax of our \emph{tagged} expressions is defined as follows:

  Figure~\ref{fig:tagged-terms-reduction} presents the syntax and semantics of an extension of the lambda calculus of the previous section with support for handling sensitivities.
  %
  Values $v$ are simple values $u$ (constants $c$ and lambdas $\lambda (x:\gty). e$)
  tagged with sensitivity information $\tg$. For now, we leave the precise definition of tags $\tg$ abstract, as it is not required to analyze the exceptional behavior of the calculus and its impact on the metatheory. Intuitively, for a literal value, this tag should be empty, and for a computed value, the tag should denote the sensitivity of the computation that produced it.\et{PB: intended sensitivity spec of a lambda? where does it come from?} For instance, $4$ as a literal constant has no sensitivity, while $4$ as the result of $x+x$ is 2-sensitive in $x$.
  %

  The operational semantics of the calculus are call-by-value, formalized using evaluation contexts, and standard save for the handling of tags.
  The novel expression $\checktag{e}[\tg]$ controls that $e$ respects a sensitivity specification $\tg$ to compute its value, and fails with an error otherwise. This behavior manifests in the reduction rule for tag-checked values: the tag of the value $t$ is {\em combined} with the expected sensitivity tag $t'$ via the (abstract) metafunction $\ttrans$. This operation either produces a new tag to be carried by the value, or is undefined, in which case an error is raised.
  %
  To reduce a function application, \et{HERE}

  first $\tg[2] \ttrans \tdom(\tg[1])$ computes a new tag for $u$, where the information in $\tg[2]$ is \emph{combined} with the information in the domain part of $\tg[1]$.
  % (obtained with $\tdom(\tg[1])$).
  This combination may not succeed if the tags contain incompatible information, in which case we raise an error.
  Then, we tag the (substituted) body with the codomain part of the tag of the argument, $\tcod(\tg[1])$.
  Same as with tags, we leave the tag meta-functions and meta-operators abstract for now.



  A primitive operation is reduced using its meta-definition $\llbracket \bop\! \rrbracket$, and a resulting tag is computed using the lifting of $\bopFuncName$ for tags, denoted by $\lceil \bopFuncName \rceil$.


  A tag-checked value is reduced by computing the tag of the inner value, $\tg \ttrans \tgp$.
  Exactly as with function applications, this combination may fail if the tags are incompatible.

  \begin{figure}[t]
  \begin{small}
  \begin{align*}
    u ::={}&
      c \mid
      \lambda (x:\gty). e
      & \syntaxLabel{simple values} \\
    %
    v ::={}& \tagged{u}
      & \syntaxLabel{tagged values}\\
    %
    e ::={}&
      v \mid
      \bop \overline{e} \mid
      x \mid
      e \app e \mid
      \checktag{e}
      & \syntaxLabel{expressions}\\
  % \end{align*}
  % \end{small}
  %
    % \begin{small}
      % \begin{align*}
        \Ectx ::={}&
          \emptycontext \mid \bop(\overline{v_i}, \Ectx, \overline{e_j}) \mid \Ectx \app e \mid v \app \Ectx \mid \checktag{\Ectx}
          & \syntaxLabel{evaluation contexts}
      \end{align*}
    \end{small}

    \textbf{Notions of reduction} \hfill
    \boxed{\ncred{e}{e}}
      \begin{small}
      \begin{align*}
          % ASCR
        %
        % \IGrefr{r-ascr} & &
        \checktag{\tagged{u}[\tg]}[\tgp]
        & \longrightarrow
        \begin{cases}
          \tagged{u}[\tg \ttrans \tgp] & \\
          \error & \text{\color{black}if not defined}
        \end{cases}\\
        %
        % APP
        %
        % \IGrefr{r-app} & &
        \tagged{(\lambda (x: \gty).e)}[\tg[1]] \app \tagged{u}[\tg[2]]
        &\longrightarrow
        \begin{cases}
          \checktag{e[\tagged{u}[\tg[2] \ttrans \tdom(\tg[1])] /x]}[\tcod(\tg[1])] \\
          \error \quad \text{\color{black} if not defined}
        \end{cases}\\
        %
        % PLUS
        %
        % \IGrefr{r-op} & &
        \bop \overline{\tagged{c_i}[\tg[i]]}
        &\longrightarrow
        \tagged{(\mathbin{\llbracket \bop\! \rrbracket}\, \overline{c_i})}[\lceil \bopFuncName \rceil(\overline{\tg[i]})]
        % %
        % % APP-SENV
        % %
        % % \IGrefr{r-inst} & &
        % \tagged{(\polyS[\r].v)}[\tg] \appS{\gsenv}
        % & \longrightarrow
        % \tagged{\substv{\gsenv}{\SG{\r}}{v}}[\tinst(\tg)]\\
        %
      \end{align*}
    \end{small}

    \textbf{\black Reduction} \hfill
    \boxed{\cred{e}{e}}

    \begin{small}

      \begin{mathpar}
        \inference{
            e_1
            \longrightarrow
            e_2
        }{
          \cred[]{
            \Ectx[][e_1]
          }{
            \Ectx[][e_2]
          }
        } \and
        \inference{
          e_1 \longrightarrow \error
        }{
          \cred[]{E[e_1]}{\error}
        }
      \end{mathpar}
    \end{small}

    \caption{Syntax and operational semantics of a tagged calculus \et{give it a name/likewise in 3}}
    \label{fig:tagged-terms-reduction}
  \end{figure}

  This operational semantics, instantiated with a good definition for tags, is designed to (1) collect a non-optimistic sound approximation of the actual sensitivity during evaluation, and (2) raise an error whenever the collected information is inconsistent.
\end{comment}


\subsection{Metric Preservation for Gradual Sensitivities}

Let us now define $\GMP$, the gradual counterpart of $\MP$.
First, we take inspiration on the gradualization of a much more known property than metric preservation: type safety.
In the gradual setting, type safety is weakened by allowing the expression of interest to error during evaluation.
As such, a gradual expression is considered type-safe if it either evaluates to a value of the correct type or halts with an error.
Consequently, $\GMP(\tenv, e, \gty, \gsenv)$---for particular environments $\denv, \venv[1], \venv[2]$ s.t. $\venvClose[\denv]{\venv[1]}{\venv[2]}$---should be of the form $\reval{\venv[1](e)}{\error} \lor \reval{\venv[2](e)}{\error} \lor (\dots)$, where $(\dots)$ is the adapted version of the conclusion of $\MP$ to the gradual setting.
\footnote{
  We define $\reval{e}{v}$ as $\creds{e}{v}[*]$, and $\reval{e}{\error}$ as $\creds{e}{\error}[*]$.
}

A naive lifting of $\MP$ to gradual sensitivities would be to simply replace $d_{\gty}(v_1, v_2) \leq \senv \cdot \denv$---the metric preservation condition for static sensitivities---by $d_{\gty}(v_1, v_2) \ccleq \gsenv \cdot \denv$.
However, such definition is problematic in many ways.
First, the dot product between $\gsenv$ and $\denv$ is now an interval, representing the minimum and maximum possible output distances.
Furthermore, comparing $d_{\gty}(v_1, v_2)$ with $\gsenv \cdot \denv$ using $\ccleq$---an optimistic operator---immediately breaks weakening of metric preservation (see Proposition~\ref{prop:sensitivity-weakening}).
For instance, suppose we know an expression is $\gsenv$-metric preserving, for $\gsenv = \sensint{0, 10}x$, which means that $d_{\gty}(v_1, v_2)$ is less than or equal to \emph{some} distance between $0$ and $10 \cdot \denv(x)$.
In particular, the actual distance may as well be the latter option.
Now consider $\gsenvp = \SG{0}x$ and notice that $\gsenv \ccleq \gsenvp$, as it is \emph{plausible} that $\SG{0}x$ is less than or equal to $\sensint{0, 10}x$.
Then, by weakening, we should be able to prove that the expression is $\gsenvp$-metric preserving.
However, this would require us to show that the measured distance is less than or equal to $0$, which is not possible in the general case.
Instead, in order to preserve weakening for the optimistic order $\ccleq$, we need to use the runtime information to obtain a non-optimistic approximation of the sensitivity of expressions.

Since expressions reduce to tagged values, we use the $\getS$ function to extract the monitored sensitivity.
Naturally, this sensitivity environment should be within the ranges proposed by $\gsenv$.
As such, inside $(\dots)$, we start checking $\reval{\venv[i](e)}{\tagged{u}[\tg[i]]} \land \getS(\tg[i]) \in \gsenv$.
Inclusion $\in$ is a the natural lifting of interval inclusion for sensitivities, \eg~$\SG{5}x + \SG{10}y \in \sensint{0,10}x + \sensint{5,15}y$ because $5 \in [0,10]$ and $10 \in [5,15]$.
Next, given that two executions may report different sensitivities, we consider the worst-case scenario.
We do this using the $\sjoin$ operator that performs the point-wise maximum of two sensitivities.
Finally, we compute the predicted output distance as $(\getS(\tg[1]) \sjoin \getS(\tg[2])) \cdot \denv$ resulting in the following conclusion:

\begin{small}
\begin{align*}
  &\reval{\venv[1](e)}{\error} \lor \reval{\venv[2](e)}{\error} \lor {}\\
  &\quad (\reval{\venv[i](e)}{\tagged{u_i}[\tg[i]]} \land \senv[i] \in \gsenv \land d_{\gty}(u_1, u_2) \leq (\senv[1] \sjoin \senv[2]) \cdot \denv) \\
  &\text{\black where} \quad \senv[i] = \getS(\tg[i])
\end{align*}
\end{small}

Reformulating it in a more succinct way, we define $\GMP$ as follows:\footnote{
  This alternative makes errors indistinguishable from other forms of non-termination, but this is not a problem for our purposes.
}

\begin{definition}[Gradual Metric Preservation]
\label{def:gsenssound}
An open expression is metric-preserving, written $\GMP(\tenv, e, \gty, \senv)$, if for all $\denv, \venv[1], \venv[2]$ such that $\venvClose[\denv]{\venv[1]}{\venv[2]}$:
\begin{small}
\begin{align*}
  &(\reval{\venv[1](e)}{v_1} \land
    \reval{\venv[2](e)}{v_2}) \implies
  d_{\gty}(v_1, v_2) \leq \senv \cdot \denv
\end{align*}
\end{small}
\end{definition}

Substitutions proximity, $\venvClose[\denv]{\venv[1]}{\venv[2]}$, is defined just as before, simply ignoring the tags of values.

Observe that, concerning termination behavior, Definition~\ref{def:gsenssound} is weaker than the one originally proposed by \citet{reedAl:icfp2010} for their static sensitivity system: if either expression fails to reduce to a value, then the relation vacuously holds, \ie~it is not necessary that the two executions have the same termination behavior; we characterize this form of gradual metric preservation as {\em termination insensitive}.
Indeed, when crafting the gradual definition, we considered that either of the two executions may fail, independent of the other.
Needless to say, a stronger alternative is possible: either both executions fail or both reduce to values at a bounded distance.
However, such definition requires a more restrictive use of imprecision.

% We now study the stronger notion of {\em termination-sensitive} gradual metric preservation.
  % While \GSoulCore does not admit divergence, \lang does feature general recursion, so we consider both divergence and runtime failures here.
% We explore sufficient conditions for \lang expressions to satisfy a stronger {\em termination-sensitive} gradual metric preservation.
  %\et{forward ref to where that's going to matter} \da{TODO: I didn't understand this; can you elaborate?}
  % Later in \secref{sec:gsoul-metatheory}, when working with \lang, which actually features general recursion, we will revisit termination-sensitive gradual metric preservation, considering both divergence and runtime failures.
  % Let us recall that we refer to non-termination as both divergence and halting with an error.
  % However, anticipating the actual presence of recursion in \lang, for this section we consider both sources of non-termination.\et{why?}


  % under an unrestricted set of assumptions over the imprecision of values and terms.
  % This has only allowed us to prove a sensitivity guarantee that cannot assure an uniform behavior of a term across different runs: the difference on the result of two executions of a  \lang term is bounded by its sensitivity only if both executions terminate, but any execution could diverge or raise an error.
  % In this section we explore how restricting the use of imprecision to be finite and stable across runs can help us stablish that a term satisfies a stronger notion of metric preservation, which we denote \emph{gradual termination-sensitive metric preservation} (gradual \TSMP \et{again, using an acronym for only one use is no good use (and I removed that unique use below)}).
  % A term in this relation presents an uniform error and divergence behavior, either always failing (or diverging) or always reducing to values at a bounded distance.

A key observation is to realize that \reviv{different termination behavior across runs} can be avoided if {\em sensitivity imprecision is finite}.
We draw from previous work \cite{dantoniAl:fpdcsl2013,toroAl:popl2019,azevedoDeAmorimAl:popl2017} to enforce the same termination behavior across runs.
Specifically, \citet{dantoniAl:fpdcsl2013} and \citet{azevedoDeAmorimAl:popl2017} show that when restricting the predicted output distance to be finite, the termination behavior of terms in their calculi is uniform.
However, this is not yet enough for our gradual language, since different substitutions may introduce values with different tags that may produce an error in only one of the executions.
Fortunately, a further restriction on the runtime information can enforce uniform termination behavior.
In their work on gradual parametricity, \citet{toroAl:popl2019} require related values to have identical runtime information to avoid errors for having more precise information in one of the executions.
%
% a stronger sensitivity guarantee, where uniformity on error and divergence is enforced.
% There are two sources of possible reduction desynchronization (either by divergence or errors) of related terms: (1) branching on $\caseKW$ terms leading to one of the terms diverging or raising an error, and (2) the presence of errors produced by different levels of precision.
%\footnote{Note that desynchronization due to divergence in gradual parametricity is not an issue, as it is not possible to relate for instance $\ttt$ with $\fff$, or $1$ with $2$.\et{why is that needed?}\mt{in case a reviewer ask why in gradual parametricity they dont have TI parametricity due divergence}}

We combine these two ideas to state a termination-sensitive gradual metric preservation.
First, we provide a new definition for substitutions proximity that requires related values to have the same tags, avoiding errors due to different levels of precision.

\begin{small}
\begin{align*}
  \venvCloseTS[\denv]{\venv[1]}{\venv[2]} \iff &
  \forall x \in \dom(\tenv).
  \Gbox{\tg[1] = \tg[2]} \land d_{\tenv(x)}(u_1, u_2) \leq \denv(x) \\
  & \text{\black where } \tagged{u_i}[\tg[i]] = \venv[i](x)
\end{align*}
\end{small}

Second, we restrict the output distance in Definition~\ref{def:gsenssound} to not be plausibly infinite.
This effectively disables the ability to branch on sensitive resources, which could lead to different termination behavior.

\begin{definition}[(Termination-sensitive) Gradual Metric Preservation]
\label{def:ts-gsenssound}
An open expression is metric-preserving, written $\GMPts(\tenv, e, \gty, \gsenv)$, if for all $\denv, \venv[1], \venv[2]$ such that $\venvCloseTS[\denv]{\venv[1]}{\venv[2]}$ and $\Gbox{\neg (\SG{\infty} \ccleq \denv \cdot \gsenv)}$:
\begin{small}
\begin{align*}
  &\reval{\venv[1](e)}{\tagged{u_1}[\tg[1]]} \ \implies \\
  & \quad
  \reval{\venv[2](e)}{\tagged{u_2}[\tg[2]]} \land
  \senv[i] \in \gsenv \land
  d_{\gty}(u_1, u_2) \leq (\senv[1] \sjoin \senv[2]) \cdot \denv
\end{align*}
\end{small}
where $\senv[i] = \getS(\tg[i])$.
\end{definition}

These two definitions of gradual metric preservation will give us a baseline for reasoning about the gradual sensitivity in our language, which we present in the next section.


==> sections/gradual_semantics.tex <==
%!TEX root = ../main.tex

\begin{figure*}
  \begin{small}
  \begin{align*}
    % Related atoms
    % (v_1, v_2) \in \glrCoreAtom{\cgty} \iff
    % & \sttyping[\emptytenv][\dom(\denv)]{v_1}{\cgty} \land \sttyping[\emptytenv][\dom(\denv)]{v_2}{\cgty} \\
    % & \ittyping{\sv[1]}{\cgty} \land \ittyping{\sv[2]}{\cgty}\\
    %
    % Related base values
    (v_1, v_2) \in \glrCoreV{\itype{\gty}{\gsenv}} \iff
    & \neg (\gsenvp \cdot \denv \cclt d_{\gty}(v_1, v_2))
    \quad \text{\textcolor{black}{where}}~ \gsenvp = \getEff(v_1) \sjoin \getEff(v_2), \gty \in \set{\rtype, \btype}\\
    % % Related numbers
    % \lrt{v_1}{\rstore[1]}{v_2}{\rstore[2]} \in \glrCoreV{\itype{\rtype}{\gsenv}} \iff
    % &
    % \neg \big( \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \lvert u_1 - u_2 \rvert \big) \quad \text{\textcolor{black}{where}}~ v_i = \evi{\itype{\rtype}{\emptysenv}, \itype{\rtype}{\gsenvp[i]}}\, u_i \ascr{\itype{\rtype}{\gsenv}}\\
    % %
    % % Related booleans
    % (v_1, v_2) \in \glrCoreV{\itype{\btype}{\gsenv}} \iff
    % &
    % \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \SG{\infty} \implies u_1 = u_2
    % \quad \text{\textcolor{black}{where}}~ v_i = \evi{\itype{\btype}{\emptysenv}, \itype{\btype}{\gsenvp[i]}}\, u_i \ascr{\itype{\btype}{\gsenv}}\\
    %
    % Related functions
    (v_1, v_2) \in \glrCoreV{\itype{(\cgty[1] \rightarrow \cgty[2])}{\gsenv}} \iff
    & \forall \svp[1], \svp[2], (v_1', v_2') \in \glrCoreV{\cgty[1]}.
     ({\sv[1] \app \svp[1]}, {\sv[2] \app \svp[2]}) \in \glrCoreT{\cgty[2] \effOp{+} \gsenv}\\
    % Related type abstractions
    (v_1, v_2) \in \glrCoreV{\itype{(\polyST.\cgty)}{\gsenv}} \iff
    & \forall \gsenvpp. ({\sv[1] \appS{\gsenvpp}}, {\sv[2] \appS{\gsenvpp}}) \in \glrCoreT{\Xisubst{\cgty}[\r]{\gsenvpp} \effOp{+} \gsenv}\\
    % Related computations
    (e_1, e_2) \in \glrCoreT{\cgty} \iff &
    (\creds[]{e_1}{\sv[1]} \land
    \creds[]{e_2}{\sv[2]}) \implies
    % (e_1 \creds v_1 \land e_2 \Downarrow v_2) \implies
    (v_1, v_2) \in \glrCoreV{\cgty}\\
     % Related environments
    (\venv[1], \venv[2]) \in \glrCoreG{\tenv} \iff
    & \dom(\venv[1]) = \dom(\venv[2]) = \dom(\Gamma) \land \forall x \in \dom(\Gamma). (\venv[1]\at{x},\venv[2]\at{x}) \in \glrCoreV{\Gamma(x)}\\
    %
    \sttyping[\tenv][\svenv]{e_1 \approx e_2}{\cgty} \iff
    & \forall \denv, \venv[1], \venv[2]. \svenv \vdash \denv \land (\venv[1], \venv[2]) \in \glrCoreG{\tenv}
      \implies (\itelabZ{\venv[1](e_1)}, \itelabZ{\venv[2](e_2)}) \in \glrCoreT{\cgty}
  \end{align*}
  \begin{align*}
    d_{\rtype}(v_1, v_2) &= \abs{\getVal(v_1) - \getVal(v_2)} &
    d_{\btype}(v_1, v_2) &= \begin{cases}
      0 & \text{if } \getVal(v_1) = \getVal(v_2)\\
      \infty & \text{otherwise}
    \end{cases}
  \end{align*}
  \end{small}
  \caption{Logical relations for gradual sensitivity soundness}
  \label{fig:basic-gradual-logical-relation}
\end{figure*}

\section{Soundness of Gradual Sensitivity Typing}
\label{sec:gradual-semantics}


We now study the main metatheoretical property of \GSoulEvCore, namely the soundness of sensitivity typing known as {\em metric preservation}~\cite{reedAl:icfp2010}.
Metric preservation is a hyperproperty that captures the bound on how much the result of two similar computations may change given an input variation, \revviii{formalized (for static functions) as follows:}

\da{Def of sensitivity/metric preservation?}
% \begin{revviiib}
% \begin{theorem}[Static metric preservation]
%   Let $f$ be a function of type $\itype{\rtype}{\r} \to \itype{\rtype}{\sensint{\sens, \sens}\r}$, for some sensitivity $\sens$.
%   Then, for any real numbers $c_1$, $c_2$ and $d$ such that $\abs{c_1 - c_2} \leq d$,
%     if $f \app c_1 \Downarrow v_1$ and $f \app c_2 \Downarrow v_2$, then $\abs{\uval{v_1} - \uval{v_2}} \leq \sens \cdot d$.
% \end{theorem}
% \end{revviiib}


\begin{ppsalb}
  In \secref{sec:gradual-metric-preservation}, we present a notion of gradual metric preservation and illustrate the key ideas of its design.
  We show that, due to possibly infinite imprecision in sensitivities, it is not possible to establish a uniform behavior for related expressions with respect to termination (either divergence or failure): gradual metric preservation is {\em termination insensitive}. In words, {\em if both expressions terminate to values}, then the difference between these values is bounded; otherwise the relation is vacuously true.\footnote{We use the term ``termination (in)sensitivity'' to concisely deal with both divergence and runtime errors---as discussed by \citet{fennellThiemann:csf2013} in the case of gradual information flow security, a runtime error can be treated as divergence.}
  Then, in \secref{sec:tsmp}, we observe that when imprecision is restricted to {\em bounded} imprecision, \ie~not plausibly infinite, \GSoulEvCore programs satisfy a stronger, \emph{termination-sensitive} gradual metric preservation: if one expression terminates to a value, then the other also terminates to a value at a bounded distance.
\end{ppsalb}

\subsection{Gradual Metric Preservation}
\label{sec:gradual-metric-preservation}

\begin{revviiib}
Figure \ref{fig:basic-gradual-logical-relation} presents our semantic model for \GSoulCore types.
The model uses a logical relation, which we use to prove metric preservation.
Due to the presence of recursive types in \lang, the full definition of the logical relation for \lang (found in the supplementary material) uses step indexing to ensure well-foundedness, albeit in a standard manner.
\end{revviiib}

The relation is defined using two mutually-defined interpretations: one for values $\glrCoreV{\cgty}$, and one for expressions $\glrCoreT{\cgty}$.
The interpretations for a type $\cgty$ are indexed by a \emph{distance environment} $\denv$.
A distance environment $\denv$ is a mapping between \revii{resources} and distances, denoted by the meta-variable $\dist$, which are syntactically equal to gradual sensitivities (making distance environments the same as gradual effects), and it represents the distance of different inputs across two different executions.
This environment is used to compute the \emph{predicted output distance} of a program, \ie~the maximum variation of the result of the program if closed by any two substitutions that satisfy the $\denv$ distances.
The predicted output distance of a program of effect $\gsenv$ is computed as $\gsenv \cdot \denv$, where $\cdot$ is the sum of the point-wise multiplication of the gradual sensitivities in $\gsenv$ and distances in $\denv$: $\gsenv \cdot \denv = \sum_{\r \in \dom(\gsenv)} \gsenv(\r) * \denv(\r)$.
Notice that the predicted output distance is a gradual interval, \ie~a range of possible distances, and it is not a single value.

In order to get an intuitive understanding of metric preservation, let us consider a simple static example.
Metric preservation allows us to reason about open programs such as $e = x+x$, which may correspond to the body of the lambda in the program $\polyS[\r]. (\lambda x: \itype{\rtype}{\r}. \Gbox{x+x})$.
In this spirit, let us choose $\Gamma = x: \r$ and $\svenv = \r$ (noticing that they effectively close the expression $e$), then $e$ has effect $\SG{2}\r$.
Consequently, if the distance environment is $\denv = \SG{3\r}$, i.e., two values of two different executions of effect $\r$ are at most at distance $\SG{3}$, then the predicted output distance is $(\SG{2\r})\cdot(\SG{3\r}) = \SG{2}*\SG{3} = \SG{6}$.
For instance, consider the following terms:

\begin{small}
  \begin{align*}
    e_1 &= (\polyS[\r]. (\lambda x: \itype{\rtype}{\r}. x+x) \app (\Gbox{1} \ascr{\itype{\rtype}{\r}})) \appS{\emptysenv} \\
    e_2 &= (\polyS[\r]. (\lambda x: \itype{\rtype}{\r}. x+x) \app (\Gbox{4} \ascr{\itype{\rtype}{\r}})) \appS{\emptysenv}
  \end{align*}
\end{small}
The expressions $e_1$ and $e_2$ will correspond to the use of two different value environments $\venv[1]$ and $\venv[2]$, such that $\venv[1] = \set{x \mapsto 1::\itype{\rtype}{\r}}$ and $\venv[2] = \set{x \mapsto 4::\itype{\rtype}{\r}}$.
Notice that both values for $x$ have effect $\r$, and are at distance $\SG{3}$, respecting both $\Gamma$ and $\denv$.
If we reduce both terms, we get $(2::\teff{\rtype}{2\r})$, and $(8::\teff{\rtype}{2\r})$, which are exactly at the predicted output distance ($\SG{6}$).
Finally, note that the expressions could have depended on multiple resources, which is already naturally supported by our logical relation.

\begin{comment}
Metric preservation also supports directly reasoning about variables that depend on multiple resources.
For instance, let us consider that in the expression $x+x$, $x$ now has effect $\SG{1}\r[1] + \SG{2}\r[2] + \SG{3}\r[3]$.
We can choose $\denv$ as $\SG{4}\r[1]+\SG{5}\r[2]+\SG{6}\r[3]$, stating that we can only close the expression with two different environments that differ in at most $4$, $5$ and $6$ for the resources $\r[1]$, $\r[2]$ and $\r[3]$, respectively.
Then, for this setting, the result can vary in at most $\SG{64}$, since $\denv \cdot \gsenv = (\SG{4\r[1]}+\SG{5\r[2]}+\SG{6\r[3]}) \cdot(\SG{2} * (\SG{1\r[1]}+\SG{2\r[2]}+\SG{3\r[3]})) = \SG{4}\cdot\SG{2}+\SG{5}\cdot\SG{4}+\SG{6}\cdot\SG{6} = \SG{64}$
\end{comment}

\paragraph{Metric Preservation in an Imprecise World}
\begin{revb}
  We write $(\sv[1],\sv[2]) \in \glrCoreV{\cgty}$ to denote that values $\sv[1]$ and $\sv[2]$ are related at type $\cgty$ and distance environment $\denv$.
  The general structure of an interpretation of some type $\cgty$, is of the form $\tilde{P}(\sv[1],\sv[2],\denv,\cgty)$, where $\tilde{P}$ is a gradual counterpart of the corresponding proposition $P$ in the static interpretation about $\sv[1]$ and $\sv[2]$ for $\denv$ and $\cgty$.
  For instance, in a static language (such as \Sax or \Fuzz), two base values are related if their distance is bounded by the predicted output distance as shown in gray:
  \begin{revviiib}
  $(v_1, v_2) \in \mathsf{static}\glrCoreV{\itype{\gty}{\gsenv}} \iff \Gbox{\gdist{\gty}(v_1, v_2) \leq \denv \cdot \gsenv}$, assuming that $\gsenv$ and $\denv$ are fully precise.\footnote{
    Note that when $\gsenv$ and $\denv$ are fully precise, the predicted output distance is a single value, thus the $\leq$ operation can be used directly.
  }
  The distance of two values is computed using the distance function $\gdist{\gty}$, which is defined for each base type $\gty$.
  For instance, $\gdist{\rtype}(v_1, v_2) = \abs{v_1 - v_2}$ and $\gdist{\btype}(v_1, v_2) = 0$ if $v_1 = v_2$ and $\infty$ otherwise.
  \end{revviiib}

  A key challenge that this work identifies in gradualizing metric preservation is that
  the gradual counterpart of this interpretation cannot just lift inequality.
  One may be tempted to define the interpretation of numbers using consistent sensitivity subtyping, interpreting the result of $\gdist{\gty}(v_1, v_2)$ as a one-point gradual sensitivity, as so:

  \begin{small}
  \begin{align*}
    {\color{red}\tikzxmark} \quad
    (n_1, n_2) \in \mathsf{naive}\glrCoreV{\itype{\gty}{\gsenv}}
    &\iff
    {\gdist{\gty}(v_1, v_2) \Gbox{\ccleq} \denv \cdot \gsenv}
  \end{align*}
  \end{small}
  Indeed, this definition is rather problematic as metric preservation is a compositional property, and so it requires to reason compositionally about value interpretations.
  In particular, given two related values, their ascriptions should yield (at least as precise) related values.
  One novel and  important consideration when designing the logical relation for values in the gradual setting is that, when lifting a predicate $P$ to its gradual counterpart, we have to reason about \emph{worst-case} scenarios for $\tilde{P}$.
  Otherwise, if we would take optimistic assumptions, one could always ascribe/refine two related values to a less sensitive type-and-effect (justified by gradual plausibility) breaking compositionality.
  To illustrate, suppose we have $(v_1, v_2) \in \mathsf{naive}\glrCoreV[\SG{1}\r]{\itype{\rtype}{\sensint{\SG{1},\SG{2}}\r}}$, where $\getVal(v_1) = 1$ and $\getVal(v_2) = 3$.
  Notice that we effectively have that $\abs{1-3} \ccleq \sensint{\SG{1},\SG{2}}$.
  Then, if we ascribe those values to $\itype{\rtype}{\SG{1}\r}$, assuming they both reduce to $v_i'$, we should have that $(v_1', v_2') \in \mathsf{naive}\glrCoreV[\SG{1}\r]{\itype{\rtype}{\SG{1}\r}}$.
  However, this is not the case, as $\abs{1-3} \ccleq \sensint{\SG{1},\SG{1}}$ does not hold.

  More technically, satisfiability of the predicate $\tilde{P}$ is not preserved after gaining precision.  % , \ie~$\forall x, x' \gprec x. \tilde{P}(x) \nRightarrow \tilde{P}(x')$.
  Consider consistent sensitivity subtyping: $2 \ccleq \sensint{\SG{1}, \SG{2}}$ is true, but $2 \ccleq \sensint{\SG{1}, \SG{1}}$ is not (and $\sensint{\SG{1}, \SG{1}} \gprec \sensint{\SG{1}, \SG{2}}$).
  For this reason, gradual metric preservation must follow a pessimistic approach, and instead {\em negate the lifting of the negated static proposition}, \ie~$\neg(\widetilde{\neg P})$.
  In particular, as $\neg (\sens[1] \leq \sens[2])$ means $\sens[2] < \sens[1]$,  we use the negation of \emph{consistently less than} defined as: $\sensint{\sens[1], \sens[2]} \cclt \sensint{\sens[3], \SG{\sens[4]}} \iff \sens[1] < \sens[4]$. Notice that proposition $\tilde{P}(x) = \neg(\gsens \cclt x)$ preserves satisfiability when $\gsens$ gains precision. And thus, in the previous example, we do not relate $\sv[1]$ and $\sv[2]$ at type $\cgty[1]$, because $\neg(\sensint{\SG{1},\SG{2}} \cclt 2)$ is false from the beginning.
  \revvi{This design requirement highlights the usefulness of using intervals, and more specifically, the lower bound of gradual sensitivities, as the distance between two values is actually compared against the lower bound of the predicted output distance.
  If the unknown sensitivity were the only form of runtime imprecision, then any time that the runtime information could not be refined to a fully-precise sensitivity, two related values would be forced to be equal (considering that the worst-case sensitivity of $\unknown$ is $\SG{0}$), making the logical relation much stricter than necessary.}

  Finally, the lifted predicates use the most precise information about types, obtained using the meta-function $\getEff$.
  Otherwise, losing precision in the type (\eg~by ascribing two related values to a very imprecise type) could break soundness.
  This can be observed in the definition of related base values, where we use the monitored sensitivity effect ($\gsenvp$, instead of $\gsenv$) to compute the predicted output distance.
  To illustrate, consider $(v_1, v_2) \in \glrCoreV{\itype{\rtype}{\SG{2}\r}}$, such that $\getVal(v_1) = 1$ and $\getVal(v_2) = 3$, thus having $\abs{1-3} \ccleq \SG{2}$.
  Then, ascribing the values to $\itype{\rtype}{\sensint{\SG{0},\SG{2}}\r}$ will not result in related values, as $\abs{1-3} \ccleq \sensint{\SG{0},\SG{2}}$ is false.
  On the contrary, if we consider only runtime information, we do not have this problem as the runtime sensitivity information of the resulting values maintain their original precision as $\SG{2} \gprec \sensint{0,2}$.
  Armed with these considerations, we now discuss each interpretation in detail.
\end{revb}

\begin{itemize}[leftmargin=*]
  \item {\em Related numbers and booleans.}
  \begin{revb}
  As explained before, two numbers are related if the difference between them is bounded by the predicted output distance.
  The same applies to booleans, with the consideration that two booleans are at distance $0$ if they are equal, and at distance $\infty$ otherwise.
  The predicted output sensitivity, is computed using $\gsenvp[1] \sjoin \gsenvp[2]$ as the (worst-case) predicted sensitivity of the values, where the effects correspond to the runtime-monitored ones, instead of the statically inferred, $\gsenv$.
  We use the join ($\sjoin$) because the precision of both effects can be different.
  The lifted predicate, $\neg (\gsenvp \cdot \denv \cclt d_{\gty}(v_1, v_2))$, can be read as requiring the distance between the two values to be less than or equal to \emph{all} values within $\gsenvp \cdot \denv$
  In other words, we do \textit{not} want a value within the output distance that is less than the difference to exist.
  %
  % For instance, consider:
  %   $v_1 = \evi{\emptysenv, \sensint{1,4}\r}\, 2 \ascr{\teff{\rtype}{\sensint{0, 10}\r}}$,
  %   $v_2 = \evi{\emptysenv, \sensint{1,5}\r}\, 5 \ascr{\teff{\rtype}{\sensint{0, 10}\r}}$ and
  %   $\denv = \SG{3\r}$. These two values belong to the interpretation $\glrCoreV{\teff{\rtype}{\sensint{0,10}\r}}$ because $\neg \big( \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \lvert u_1 - u_2 \rvert \big) = \neg \big( (\SG{3\r}) \cdot (\SG{\sensint{1,4}\r} \sjoin \SG{\sensint{1,5}\r}) \cclt \lvert 2 - 5 \rvert \big) \iff \neg \big( \sensint{3,15} \cclt \SG{3} \big)$ holds.
  \end{revb}


  \item {\em Related functions and resource abstractions.}
  \rev{
    Two functions or resource abstractions are related if their applications to two related arguments or a sensitivity effect, respectively, yield related computations.
  }

  \item \emph{Related expressions.}
  A pair of expressions are related if they both reduce to values, and those two values are related.
  Observe that this definition is weaker than the one originally proposed by \citet{reedAl:icfp2010}: if either expression does not reduce to a value, then the relation vacuously holds; we say that gradual metric preservation is {\em termination insensitive}.
  The easiest way to see this is to close an expression with two different substitutions $\venv[1]$ and $\venv[2]$, such that $\venv[1] \gprec \venv[2]$.
  Having that $\venv[1](e)$ is more precise, it is possible that $\venv[1](e)$ results in an error, while $\venv[2](e)$ does not.
  % One simple example of an expression that behaves differently (in terms of termination) when closed by different substitutions is the expression
  %   $e = \ev x \ascr{\itype{\rtype}{\sensint{2,3}\r}}$, where
  %   $\ev = \evi{\itype{\rtype}{\sensint{2,3}\r}, \itype{\rtype}{\sensint{2,3}\r}}$.
  % If we close it with
  %   $\venv[1] = \set{x \mapsto \ev[1] 1::\itype{\rtype}{\sensint{1,2}\r}}$ and
  %   $\venv[2] = \set{x \mapsto \ev[2] 1::\itype{\rtype}{\sensint{1,2}\r}}$, where
  %   $\ev[1] = \evi{\teff{\rtype}{\emptysenv},\teff{\rtype}{1\r}}$ and
  %   $\ev[2] = \evi{\teff{\rtype}{\emptysenv},\teff{\rtype}{\sensint{1,2}\r}}$,
  %   then $\venv[1](e)$ will halt with an error, while $\venv[2](e)$ will not.
  % Notice that the only difference between $\venv[1]$ and $\venv[2]$ is the precision of evidences, having $\ev[1] \transsub \ev$ being undefined, in contrast to $\ev[2] \transsub \ev$ which evaluates to $\ev$ (as no precision is gained).
  %diverges (or errors).
  % Thus, there is no way to guarantee that the second term will terminate, when the first one has terminated.
  We come back to this aspect in \secref{sec:tsmp}.
  % we come back to this issue and propose a solution\et{bad pitch (see zulip from friday)} to avoid desynchronization by restricting sensitivity information to be finite \et{finitely imprecise?} and equal for related values.


  \item \emph{Related substitutions.}
  Two substitutions are related at type environment $\Gamma$, if each variable in common, $x$, is bound to related values at type $\Gamma(x)$.
\end{itemize}


Lastly, to state the main relation, we say that a distance environment is well-formed w.r.t. a resources set, written $\svenv \vdash \denv$, if it closes all the resources in the set, \ie~$\dom(\denv) \subseteq \svenv$.

\begin{itemize}[leftmargin=*]
  \item \emph{Related \GSoulCore expressions.}
  Two open expressions are related, written $\sttyping[\tenv][\svenv]{e_1 \approx e_2}{\cgty}$, if for any distance environment $\denv$ well formed w.r.t $\svenv$, and any two related substitutions $\venv[1], \venv[2]$, the computations of the expressions closed by $\venv[1]$ and $\venv[2]$ are related.
\end{itemize}

% we need notions of well-formedness of environments so they can be used to close and compute the predicted output distance of a term.
% These are based on the meta-functions $\freevars{\cdot}$ and $\freesvars(\cdot)$ (defined in the supplementary material), which return the free variables and free resources of a term, respectively.
%  % of a type environment with respect to a term\revii{, and well-formedness of a distance environment with respect to a type environment}:

% % \begin{definition}[Type environment well-formedness]
% %   A type environment $\tenv$ is well-formed with respect to an intrinsic term $t$, denoted $t \vdash \tenv$ if and only if
% %   $\freevars{t} \subseteq \dom(t)$ and $\forall x^{\cgty} \in \freevars{t}.~ \tenv(x) = \cgty$.
% % \end{definition}

% \begin{reviib}
% \begin{definition}[Distance environment well-formedness]
%   Well-formedness of a distance environment $\denv$ with respect to a type environment $\tenv$, denoted $\tenv |- \denv$, is defined as follows:
%   \begin{mathpar}
%   \inference{}{\emptyenv |- \denv} \and
%   \inference{\tenv |- \denv & \freesvars(\cgty) \subseteq \dom(\denv)}{\tenv, x:\cgty |- \denv}
%   \end{mathpar}
% \end{definition}

% % These two definitions capture the requirement that every resource used in $\tenv$, well-formed with respect to $t$, should also be defined in $\denv$. Otherwise, $\denv$ could not be used to compute the predicted output distance of term $t$, as operation $\denv \cdot \gsenv$ would not be fully defined.
% % must be defined for every $\gsenv$ found in types and evidences of $t$.
% \end{reviib}

\paragraph{Soundness of \GSoulEvCore}
As usual, for logical relations, soundness of the type system is established as the fundamental property of the logical relation: if an open expression typechecks, then it is related to itself.

\begin{revb}
\begin{restatable}[Fundamental Property]{theorem}{gradualMetricPreservation}
  \label{prop:gradual-metric-preservation}
  If $\sttyping[\tenv][\svenv]{e}{\cgty}$, then $\sttyping[\tenv][\svenv]{e \approx e}{\cgty}$.
  % For any $\denv$ such that $\svenv \vdash \denv$, and any $(\venv[1], \venv[2]) \in \glrCoreG{\tenv}$, we have $(\lceil \venv[1](e) \rceil, \lceil \venv[2](e) \rceil) \in \glrCoreT{\cgty}$.
  % \reviv{Let $t$ be a \GSoulEvCore term.}
  % If $\ittyping{t}{\cgty}$ and $t \vdash \tenv$,
  % then $\forall \denv, \venv[1], \venv[2]$ such that $\tenv \vdash \denv$ and $(\venv[1], \venv[2]) \in \glrCoreG{\tenv}$,
  % we have $(\venv[1](t), \venv[2](t)) \in \glrCoreT{\cgty}$.
\end{restatable}
\end{revb}


% \begin{restatable}[Gradual metric preservation]{corollary}{gradualMetricPreservationtt}
%   \label{prop:gradual-metric-preservationtt}
%   If $\ittyping{t}{\cgty}$ and $t \vdash \tenv$,
%   then $\forall \denv, k\geq0, \venv[1], \venv[2]$ such that $\tenv \vdash \denv$ and $(\venv[1], \venv[2]) \in \glrCoreG{\tenv}$,
%   we have $\forall j < k$,
%     $\creds[{\venv[1]}]{t_1}{\sv[1]}[j]$ and $\creds[{\venv[2]}]{t_2}{\sv[2]}$ implies that $
%     (v_1, v_2) \in \glrCoreV{\cgty}[k-j]$.
% \end{restatable}

In particular we have the following metric preservation result for base types:\footnote{
  Notation $\pi_2(\gsens)$ gets the upper bound of a sensitivity interval, \ie~$\pi_2(\sensint{a,b}) = b$.
}

\begin{restatable}[Gradual metric preservation for base types]{corollary}{gradualMetricPreservationBaseTypes}
  \label{prop:gradual-metric-preservation-base-types}
  Let $f$ be a \GSoulCore function of type $\teff{\rtype}{\r} -> \teff{\rtype}{\gsens \r}$.
  For any real numbers $c_1, c_2, d$ such that $\abs{c_1 - c_2} \leq d$,
  if $\reval{f \app c_1}{v_1}$ and $\reval{f \app c_2}{v_2}$, then
  $\abs{\uval{v_1} - \uval{v_2}} \leq \pi_2(\gsens) \cdot d$.
\end{restatable}
Notice that this result is not as strong as the fundamental property, but it captures the expected static source level guarantee: the observed difference between values is bounded using the upper bound of the specified sensitivity interval.
In contrast, the logical relations use the monitored lower bound of the sensitivity effect.

% \et{missing connection between T4 and C5 (different languages)}


\begin{comment}
\paragraph{\revii{Example of gradual metric preservation}.}
% \mt{This is candidate to be removed if we don't have space} \et{could compact the presentation as well}
Let $t = \ev[2] (x + (\ev[1] 1 \ascr{\teff{\rtype}{\unknown x}})) \ascr{\teff{\rtype}{\sensint{0,2}x}}$, where
  $\ev[1] = \evi{\teff{\rtype}{\emptysenv}, \teff{\rtype}{\unknown x}}$ and
  $\ev[2] = \evi{\teff{\rtype}{1x}, \teff{\rtype}{\sensint{1, 2}x}}$.
Consider
  $\tenv = x: \teff{\rtype}{x}$,
  $\denv = \SG{2x}$,
  $\venv[1] = \set{x \mapsto \evi{\itype{\rtype}{\emptysenv}, \teff{\rtype}{x}}\, 4 \ascr{\teff{\rtype}{x}}}$ and
  $\venv[2] = \set{x \mapsto \evi{\itype{\rtype}{\emptysenv}, \teff{\rtype}{x}}\, 5 \ascr{\teff{\rtype}{x}}}$.

Let us establish that $(\venv[1], \venv[2]) \in \glrCoreG{\tenv}$:
\revii{
\begin{enumerate}
\item $\dom(\tenv) = \dom(\venv[1]) = \dom(\venv[2])$ is trivial, and
\item $(\evi{\itype{\rtype}{\emptysenv}, \teff{\rtype}{x}} 4 \ascr{\teff{\rtype}{x}}, \evi{\itype{\rtype}{\emptysenv}, \teff{\rtype}{x}} 5 \ascr{\teff{\rtype}{x}}) \in \glrCoreV{\teff{\rtype}{x}}$, because,  $\neg (\SG{2x}\cdot(\SG{1x} \sjoin \SG{1x}) \cclt |4-5|) \iff \neg (2 \cclt 1) \iff \top$.
\end{enumerate}
}

Then by Proposition \ref{prop:gradual-metric-preservation} we know that $(\itconfig[\venv[1]]{t}, \itconfig[\venv[2]]{t}) \in \glrCoreT{\teff{\rtype}{\sensint{0,2}x}}$. Let us see why:
\begin{itemize}
  \item Suppose $\creds[\venv[1]]{t}{\ev\, 5 \ascr{\teff{\rtype}{\sensint{0,2}x}}}[j]$, for some $j<k$, where $\ev = \evi{\itype{\rtype}{\emptysenv}, \teff{\rtype}{\sensint{1,2}x}}$. Analogously, $\creds[\venv[2]]{t}{\ev\, 6 \ascr{\teff{\rtype}{\sensint{0,2}x}}}$.
  \item $(\ev 5 \ascr{\teff{\rtype}{\sensint{0,2}x}}, \ev 6 \ascr{\teff{\rtype}{\sensint{0,2}x}}) \in \glrCoreV{\teff{\rtype}{\sensint{0,2}x}}[k-j]$: $\neg \big( (\SG{2x}) \cdot (\SG{\sensint{1,2}x} \sjoin \SG{\sensint{1,2}x}) \cclt \lvert 5 - 6 \rvert \big) \iff \neg \big( \sensint{2,4} \cclt \SG{1} \big)$, which is true.
  % \begin{align*}
  %   \neg \big( (2x) \cdot (\sensint{1,2}x \sjoin \sensint{1,2}x) \cclt \lvert 5 - 6 \rvert \big)
  %   &\iff \neg \big( (2x) \cdot (\sensint{1,2}x) \cclt \lvert 5 - 6 \rvert \big)\\
  %   &\iff \neg \big( \sensint{2,4} \cclt 1 \big)\\
  %   &\iff \neg \big( \bot \big)\\
  %   &\iff \top\\
  % \end{align*}
\end{itemize}
\end{comment}

% \et{why is this here?} Type safety and soundness for \lambdaSens{} are specific cases of the \lang{} theorems, so their proofs are corollaries of the properties presented in this section.

\begin{ppsalb}
  \subsection{Termination-Sensitive Gradual Metric Preservation}
  \label{sec:tsmp}

We now study the stronger notion of {\em termination-sensitive} gradual metric preservation.
  While \GSoulCore does not admit divergence, \lang does feature general recursion, so we consider both divergence and runtime failures here.
% We explore sufficient conditions for \lang expressions to satisfy a stronger {\em termination-sensitive} gradual metric preservation.
  %\et{forward ref to where that's going to matter} \da{TODO: I didn't understand this; can you elaborate?}
  % Later in \secref{sec:gsoul-metatheory}, when working with \lang, which actually features general recursion, we will revisit termination-sensitive gradual metric preservation, considering both divergence and runtime failures.
  % Let us recall that we refer to non-termination as both divergence and halting with an error.
  % However, anticipating the actual presence of recursion in \lang, for this section we consider both sources of non-termination.\et{why?}


  % under an unrestricted set of assumptions over the imprecision of values and terms.
  % This has only allowed us to prove a sensitivity guarantee that cannot assure an uniform behavior of a term across different runs: the difference on the result of two executions of a  \lang term is bounded by its sensitivity only if both executions terminate, but any execution could diverge or raise an error.
  % In this section we explore how restricting the use of imprecision to be finite and stable across runs can help us stablish that a term satisfies a stronger notion of metric preservation, which we denote \emph{gradual termination-sensitive metric preservation} (gradual \TSMP \et{again, using an acronym for only one use is no good use (and I removed that unique use below)}).
  % A term in this relation presents an uniform error and divergence behavior, either always failing (or diverging) or always reducing to values at a bounded distance.

  A key observation is to realize that \reviv{different termination behavior across runs} can be avoided if {\em sensitivity imprecision is finite}.
  We draw from \citet{dantoniAl:fpdcsl2013} and \citet{toroAl:popl2019} to enforce the same behavior of divergence and failures between runs, respectively.
  Specifically, \citet{dantoniAl:fpdcsl2013} restrict the definition of metric preservation to only reason about finite distances, effectively disallowing the different behaviors of reduction due to conditionals and case analysis; and in their work on gradual parametricity, \citet{toroAl:popl2019} require related values to have identical runtime information to avoid errors for having more precise information in one of the executions.
  %
  % a stronger sensitivity guarantee, where uniformity on error and divergence is enforced.
  % There are two sources of possible reduction desynchronization (either by divergence or errors) of related terms: (1) branching on $\caseKW$ terms leading to one of the terms diverging or raising an error, and (2) the presence of errors produced by different levels of precision.
  %\footnote{Note that desynchronization due to divergence in gradual parametricity is not an issue, as it is not possible to relate for instance $\ttt$ with $\fff$, or $1$ with $2$.\et{why is that needed?}\mt{in case a reviewer ask why in gradual parametricity they dont have TI parametricity due divergence}}

  We combine these two ideas to state a termination-sensitive gradual metric preservation. \begin{revivb}
  Figure~\ref{fig:ts-gradual-logical-relation} presents the new definitions for related values and open expressions, along with a termination-sensitive characterization of related expressions.
  First, we add an additional requirement to all value relations definitions: both values must have the same runtime information, preventing one execution from failing while the other does not due to higher precision in one of the executions.
  We perform this check using the $\getRT$ function, which extracts the runtime information from a value.
  \footnote{Notice that the runtime information also includes information about the effects contained inside the type of the value, not only the top-level effect.
  Hence why we use the $\getRT$ function instead of just comparing the top-level effects through the $\getEff$ function.}
  We use a new definition for related terms in which the reduction of the second term is in the right-hand side of the implication, ensuring that both executions have the same termination behavior.
  And finally, we add a new restriction to the definition of related \GSoulCore expressions: the output distance cannot plausibly be $\SG{\infty}$, as this would allow both executions to branch differently, leading to different termination behavior.

  \begin{figure}
  \begin{small}
    \begin{align*}
      % Related atoms
      (v_1, v_2) \in \tsglrV{\cgty}[] \iff
      % & \ittyping{\sv[1]}{\cgty} \land \ittyping{\sv[2]}{\cgty} \land {}\\
      & \Gbox{\getRT(v_1) = \getRT(v_2)} \land \dots \\
      % Related terms
      (t_1, t_2) \in \tsglrT{\cgty}[] \iff
      & \creds[]{t_1}{v_1} \implies (\Gbox{\exists v_2 . \creds[]{t_2}{v_2}[*]} \land {} \\ & (v_1, v_2) \in \tsglrV{\cgty}[])\\
      \sttyping[\tenv][\svenv]{e_1 \approx_{\mathsf{ts}} e_2}{\cgty}
      \iff
      & \forall \denv, \venv[1], \venv[2]. (\svenv \vdash \denv \land {} \\
      & \Gbox{\neg (\SG{\infty} \ccleq \eff(\cgty) \cdot \denv)} \land {}\\
      & (\venv[1], \venv[2]) \in \tsglrG{\tenv}[]) \implies  {}\\
      & (\itelabZ{\venv[1](e_1)}, \itelabZ{\venv[2](e_2)}) \in \tsglrT{\cgty}[]
    \end{align*}
  \end{small}

  \caption{Termination-sensitive gradual metric preservation}
  \label{fig:ts-gradual-logical-relation}
  \end{figure}

  \begin{restatable}[(Termination-sensitive) Fundamental Property]{theorem}{tsgradualMetricPreservation}
    \label{prop:ts-gradual-metric-preservation}
    If $\sttyping[\tenv][\svenv]{e}{\cgty}$, then $\sttyping[\tenv][\svenv]{e \approx_{\mathsf{ts}} e}{\cgty}$.
    % Suppose $\sttyping[\tenv][\svenv]{e}{\itype{\gty}{\gsenv}}$, then for any $\denv$ such that $\svenv \vdash \denv$ and $\Gbox{\neg (\SG{\infty} \ccleq \denv \cdot \gsenv)}$, and any $(\venv[1], \venv[2]) \in \tsglrG{\tenv}[]$, we have $(\venv[1](e), \venv[2](e)) \in \tsglrT{\itype{\gty}{\gsenv}}[]$.
    % \reviv{
    %   Let $t$ be a \GSoulEvCore term.
    % }
    % If $\ittyping{t}{\itype{\gty}{\gsenv}}$, $t \vdash \tenv$ and $\Gbox{\neg (\SG{\infty} \ccleq \denv \cdot \gsenv)}$,
    % then $\forall \denv, \venv[1], \venv[2]$ such that $\tenv \vdash \denv$ and $(\venv[1], \venv[2]) \in \tsglrG{\tenv}[]$,
    % we have $(\venv[1](t), \venv[2](t)) \in \tsglrT{\itype{\gty}{\gsenv}}[]$.
  \end{restatable}
  \end{revivb}

  \revvi{
  Notice that for imprecise terms, this result is only useful due to the availability of sensitivity intervals, as the presence of $\unknown$ in the top-level type trivially makes the condition $\neg (\SG{\infty} \ccleq \denv \cdot \gsenv)$ false.}
  Finally, the two extra conditions are sufficient to establish termination-sensitive gradual metric preservation, as captured in the following corollary.
  % that if the first term reduces to a value, then the second also reduces to a value.

  % \begin{restatable}[Termination-sensitive gradual metric preservation]{theorem}{gradualTSMetricPreservation}
  %   \label{prop:ts-gradual-metric-preservation}
  %   If $\ittyping{t}{\itype{\gty}{\gsenv}}$ and $t \vdash \tenv$,
  %   then $\forall \denv, k \geq 0, \venv[1], \venv[2]$ such that
  %   $\tenv \vdash \denv$, $(\venv[1], \venv[2]) \in \tsglrG{\tenv}$ and $\neg (\infty \ccleq \denv \cdot \gsenv)$, we have $(\itconfig[\venv[1]]{t}, \itconfig[\venv[2]]{t}) \in \tsglrT{\itype{\gty}{\gsenv}}$.
  % \end{restatable}

  \begin{restatable}[(Termination-sensitive) gradual metric preservation for base types]{corollary}{gradualMetricPreservationBaseTypesTS}
    \label{prop:gradual-metric-preservation-base-types-TS}
    \reviv{Let $f$ be a \GSoulCore function.}
    Let $f$ be a function of type $\teff{(\teff{\rtype}{\r} -> \teff{\rtype}{\gsens \r})}{\emptysenv}$.
    For any real numbers $c_1, c_2, d$ such that $\abs{c_1 - c_2} \leq d$ and $\pi_2(\gsens) \cdot d < \infty$,
    if $\reval{f \app c_1}{v_1}$ then
    $\reval{f \app c_2}{v_2}$ and
    $\abs{\uval{v_1} - \uval{v_2}} \leq \pi_2(\gsens) \cdot d$.
  \end{restatable}

  The difference between Corollary~\ref{prop:gradual-metric-preservation-base-types} and Corollary~\ref{prop:gradual-metric-preservation-base-types-TS} is that in the latter, the overall distance of the outputs $\pi_2(\gsens) \cdot d$ cannot plausibly be infinite. Consequently, the result is termination sensitive.
  The fact that this stronger guarantee holds for \GSoulCore expressions whose imprecision is restricted to be finite illustrates how the progressive hardening of imprecision can lead to stronger guarantees.
  We observe that this should encourage programmers to use bounded imprecision whenever possible, which we see as a strong motivation for supporting sensitivity intervals in gradual source sensitivity languages.
\end{ppsalb}


==> sections/gradual_sens.tex <==
%!TEX root = ../main.tex
\section{\GSoulCore: Gradual Sensitivity Typing}
\label{sec:gradual-lang}




\mt{HERE}


\begin{revvib}
We now present \GSoulCore, a core language with gradual sensitivity typing and subset of \lang, \et{rewrite:} which supports functions, explicit resource polymorphism and ascriptions.
\GSoulCore captures the interesting aspects and challenges of gradual sensitivity typing, while \lang is a practical language with additional constructs such as sum, product, and recursive types.
%, which we later extend to \lang (\S\ref{sec:extensions}).
% , which we design following the principles of the Abstracting Gradual Typing (AGT) framework~\cite{garciaAl:popl2016}. \da{TODO: summary of the section}.
We use {\color{StoreGreen} green} for sensitivity related variables, and {\color{EqBlue}blue} for the rest of the math notation.
\rev{
  The semantics of the language are initially based on \Sax~\cite{toroAl:toplas2023} and its latent type-and-effect discipline, here extended with ascriptions and explicit resource polymorphism.}\footnote{Both \GSoulCore and \lang are crafted by following the principles of the Abstracting Gradual Typing methodology~\cite{garciaAl:popl2016}.
However, this paper focuses on the salient aspects of the language, and does not detail the gradualization process, given the space restriction and the fact that the application of AGT to various disciplines is well-documented in the literature~\cite{garciaAl:popl2016,toroTanter:scp2020,toroAl:toplas2018,toroAl:popl2019,lehmannTanter:popl2017,malewskiAl:oopsla2021,toroTanter:tr2017}.
For the curious reader, we do describe a static sensitivity language, \lambdaSens, and the technical details of its AGT-driven gradualization, \lang, in the supplementary material. \da{Keep this?}}
\end{revvib}

\subsection{Syntax}
% \begin{figure}[t]
%   \begin{small}
%   % \begin{mathpar}
%   %   c \in \rtype \cup \btype, \quad
%   %   x \in \VarClass, \quad
%   %   e \in \ExprClass, \quad
%   %   \r \in \ResClass, \quad
%   %   \gsens \in \GSensClass, \\
%   %   \gsenv \in \GSenvClass, \quad
%   %   \gty \in \GTyClass, \quad
%   %   \cgty \in \GTypeClass
%   % \end{mathpar}
%   \begin{align*}
%     % \gsens  ::= {}& \sensint{\sens, \sens} %\quad (\text{\color{black}with sugar } \unknown \triangleq \sensint{0, \infty} \text{ \color{black}and } \sens \triangleq \sensint{\sens, \sens})
%     % & \syntaxLabel{gradual sensitivities}\\
%     %
%     \gsenv  ::= {}& \SG{\gsens \r + \dots + \gsens \r} & \syntaxLabel{sensitivity effects}\\
%     %
%     \Bty   ::= {}& \rtype \mid \btype & \syntaxLabel{base \tyclsPlur}\\
%     \gty    ::= {}&
%       \Bty \mid
%       \cgty \rightarrow \cgty \mid
%       \polyST . \cgty
%       & \syntaxLabel{\tyclsPlur{}}\\
%     \cgty   ::= {}&
%       \itype{\gty}{\gsenv}
%       & \syntaxLabel{\typeclsPlur{}}\\
%     e ::= {}&
%       c \mid \bop \overline{e} \mid
%       x \mid \lambda (x:\cgty). e \mid e \app e
%       & \syntaxLabel{expressions} \\
%       &\mid \polyS[\r]. e \mid
%       e \appS{\gsenv} \mid e \ascr{\cgty}
%   \end{align*}
%   \end{small}
%   \caption{Syntax of Gradual Sensitivity Types\et{not only types}}
%   \label{fig:syntax-gsens}
% \end{figure}
The \reviv{syntax} of \GSoulCore is presented in Figure~\ref{fig:syntax-gsens}.
\begin{comment}
We aim to support imprecision only in the sensitivity parts of the type system.
Therefore, the \quot{dynamic} end of the spectrum is simply typed.
\end{comment}
As explained and illustrated in \S\ref{sec:in-action}, we support both unbounded imprecision via the fully-unknown sensitivity $\unknown$ and bounded imprecision via sensitivity intervals such as $\sensint{1, 2}$.
A gradual sensitivity $\gsens$ is defined as a valid interval of two static sensitivities. % where the lower bound is less than or equal to the upper bound.
A sensitivity $\sens$ is a positive real number or infinity, where $\sinfty \cdot \SG{0} = \SG{0} \cdot \sinfty = \SG{0}$ and $\sens \cdot \sinfty = \sinfty \cdot \sens = \sinfty$ if $\sens > \SG{0}$.
This way, a gradual sensitivity captures the plausibility of a sensitivity being any number within the range.
Finally, the unknown sensitivity $\unknown$ is just syntactic sugar for the interval $\sensint{0, \infty}$, and a \textit{fully precise} sensitivity $\sens$ is sugar for the interval $\sensint{\sens,\sens}$.
For example, the gradual sensitivities $\sensint{0, \infty}$ and $\sensint{3, 3}$ can also be written as $\unknown$ and $\sensval{3}$, respectively.

\et{first, introduce the notion of resource / resource variable -- the basics is that GSCore is about tracking sensitivity s about resources r. Start with that: we have a lambda calculus + primitive ops + resources and track sensitivity} Sensitivity effects, characterized by the meta-variable $\gsenv$, are mappings between resource variables $\r$ and gradual sensitivities $\gsens$.
For simplicity we write effects as first-order polynomials, \eg~$\gsenv = \SG{\r[1] + \unknown\r[2]}$ is a sensitivity effect where $\gsenv(\SG{\r[1]}) = \SG{1}$, $\gsenv(\SG{\r[2]}) = \unknown$\revii{, and $\gsenv(\r) = \SG{0}$ for any other resource $\r$ in scope}.
Across the paper, we use $\r$ (written in \SG{green}) for resource variables.

A \tyclsSing{} $\gty$ can be the real number type $\rtype$, \reviv{the boolean type $\btype$,} a function type $\cgty \rightarrow \cgty$, or a \reviv{resource} quantification $\polyST. \cgty$.
The latter is a type that abstracts over a resource variable $\r$ in the body $\cgty$.
A type-and-effect $\cgty$ is a tuple $\itype{\gty}{\gsenv}$ associating a type $\gty$ and a sensitivity effect $\gsenv$. \mt{remove?} Note that, function types are of the form $\itype{(\itype{\gty[1]}{\gsenv[1]} \rightarrow \itype{\gty[2]}{\gsenv[2]})}{\gsenv}$  where $\gsenv[1]$ is the expected effect of the argument, $\gsenv[2]$ is called the \textit{latent effect} of the produced function and $\gsenv$ is the effect of evaluating the expression  \da{cite Toro et al. on latent effects?}.

Expressions $e$ include \reviv{constants, primitive operations}, variables, lambda expressions, applications, \rev{resource abstractions, sensitivity effect applications,} and ascriptions.
In contrast to resource variables, we use meta-variables $x, y, z$ (written in {\color{EqBlue}blue}) for lambda-bound variables.
\revviii{
In contrast to previous work~\cite{reedAl:icfp2010,nearAl:oopsla2010,toroAl:toplas2023}, resources are explicitly introduced using resource abstraction $\polyS[\r]. e$, where the resource variable $\r$ is bound in the body $e$.
For instance, the resource-polymorphic function that doubles its argument can be written as \mbox{$\polyS[\r]. \lambda (x: \teff{\rtype}{\r}). x + x$}.
Dually, a sensitivity effect application $e \appS{\gsenv}$ eliminates a resource variable $\r$ with a sensitivity effect $\gsenv$.
Finally, ascriptions, written $e \ascr{\cgty}$, are used to statically\et{well, not fully} enforce a type-and-effect on an expression.
}

\et{new section follows -- that's not about the syntax anymore}

\begin{figure*}
  \begin{small}
  \begin{align*}
    % Related atoms
    % (v_1, v_2) \in \glrCoreAtom{\cgty} \iff
    % & \sttyping[\emptytenv][\dom(\denv)]{v_1}{\cgty} \land \sttyping[\emptytenv][\dom(\denv)]{v_2}{\cgty} \\
    % & \ittyping{\sv[1]}{\cgty} \land \ittyping{\sv[2]}{\cgty}\\
    %
    % Related base values
    (v_1, v_2) \in \glrCoreV{\itype{\Bty}{\gsenv}} \iff
    &
    v_i \in \llbracket \Bty \rrbracket \land
     \neg (\gsenvp \cdot \denv \cclt d_{\Bty}(v_1, v_2))
    \quad \text{\textcolor{black}{where}}~ \gsenvp = \getEff(v_1) \sjoin \getEff(v_2)\\
    % % Related numbers
    % \lrt{v_1}{\rstore[1]}{v_2}{\rstore[2]} \in \glrCoreV{\itype{\rtype}{\gsenv}} \iff
    % &
    % \neg \big( \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \lvert u_1 - u_2 \rvert \big) \quad \text{\textcolor{black}{where}}~ v_i = \evi{\itype{\rtype}{\emptysenv}, \itype{\rtype}{\gsenvp[i]}}\, u_i \ascr{\itype{\rtype}{\gsenv}}\\
    % %
    % % Related booleans
    % (v_1, v_2) \in \glrCoreV{\itype{\btype}{\gsenv}} \iff
    % &
    % \denv \cdot (\gsenvp[1] \sjoin \gsenvp[2]) \cclt \SG{\infty} \implies u_1 = u_2
    % \quad \text{\textcolor{black}{where}}~ v_i = \evi{\itype{\btype}{\emptysenv}, \itype{\btype}{\gsenvp[i]}}\, u_i \ascr{\itype{\btype}{\gsenv}}\\
    %
    % Related functions
    (v_1, v_2) \in \glrCoreV{\itype{(\cgty[1] \rightarrow \cgty[2])}{\gsenv}} \iff
    & \forall \svp[1], \svp[2], (v_1', v_2') \in \glrCoreV{\cgty[1]}.
     ({\sv[1] \app \svp[1]}, {\sv[2] \app \svp[2]}) \in \glrCoreT{\cgty[2] \effOp{+} \gsenv}\\
    % Related type abstractions
    (v_1, v_2) \in \glrCoreV{\itype{(\polyST.\cgty)}{\gsenv}} \iff
    & \forall \gsenvpp. ({\sv[1] \appS{\gsenvpp}}, {\sv[2] \appS{\gsenvpp}}) \in \glrCoreT{\Xisubst{\cgty}[\r]{\gsenvpp} \effOp{+} \gsenv}\\
    % Related computations
    (e_1, e_2) \in \glrCoreT{\cgty} \iff &
    (\creds[]{e_1}{\sv[1]} \land
    \creds[]{e_2}{\sv[2]}) \implies
    % (e_1 \creds v_1 \land e_2 \Downarrow v_2) \implies
    (v_1, v_2) \in \glrCoreV{\cgty}\\
     % Related environments
    (\venv[1], \venv[2]) \in \glrCoreG{\tenv} \iff
    & \
    % dom(\venv[1]) = \dom(\venv[2]) = \dom(\Gamma) \land
    \forall x \in \dom(\Gamma). (\venv[1]\at{x},\venv[2]\at{x}) \in \glrCoreV{\Gamma(x)}\\
    %
    \semtyping[\tenv][\svenv]{e}{\cgty} \iff
    & \forall \denv, \venv[1], \venv[2]. \svenv \vdash \denv \land (\venv[1], \venv[2]) \in \glrCoreG{\tenv}
      \implies ({\venv[1](e)}, {\venv[2](e)}) \in \glrCoreT{\cgty}
  \end{align*}
  \begin{align*}
    d_{\rtype}(v_1, v_2) &= \abs{\getVal(v_1) - \getVal(v_2)} &
    d_{\btype}(v_1, v_2) &= \begin{cases}
      0 & \text{if } \getVal(v_1) = \getVal(v_2)\\
      \infty & \text{otherwise}
    \end{cases}
  \end{align*}
  \end{small}
  \caption{Logical relations for gradual sensitivity soundness}
  \label{fig:basic-gradual-logical-relation}
\end{figure*}
\begin{revviiib}
Figure \ref{fig:basic-gradual-logical-relation} presents our semantic model for \GSoulCore types.
The model is preseted using binary logical relations, which we exploit later to prove soundness (metric preservation).
\end{revviiib}

\et{start with the big picture: we're tracking sensitivity, so we're baking it in the meaning of types. focus on the base type case first and maintain/make explicit the intuition with the lipschitz continuity definition, recall it, and explain how it's scaled up to talk about n resources}

\begin{revviiib}
The logical relation is mutually defined interpretation for values and computations.
The value relation is indexed by ... and a type-and-effect... Delta represents ...., for instance....
The value relation ... defines, for each type, which
values (at which worlds and step-indices) lie in that type.
A value $v$ is ....
Two constants values ($v_1$, $v_2$) are related at base type $g$ and effect $\Sigma$, if (1) both constants are syntactic values of type $g$, $v_i \in \llbracket g \rrbracket$, and their predicted output distance, written $\Sigma' \cdot \Delta$ is not plausible smaller than the actual distance between the values. To compute Sigma' we use metafunction ... and we take the worst case using the join operation according to the lattice of sensitivity.
To compute the distance,  we use metafunction ... to compute the distance for reals and booleans respectively, and we use ... to extract the runtime effect of a value.


The interpretation for function types and effect are the set of pair of values, that given pair of related arguments, their application yield related computations. We use $+$ operator to ``add'' the effect of the lambda to the effect of the body of the function.

The interpretation for resource quantification and effect are the set of pair of values, their instantiation to any effect yield related computation at ... We use $[\Sigma/x]G$ to denote the substitution of $x$ for $\Sigma$ in $G$. Note that we also use $+$ to add the effect of the abstraction to the effect of its body $G$.

Finally, the semantic model for computations at type-and-effect $G$ are the pair of expressions that if they both reduce to values, then the values are related at the given type-and-effect. We use notation $e \mapsto v$ to denote that $e$ reduces to $v$ in some number of steps. The formal definition is presented in ... below.

Continue with $\gamma$, and then the semantic of typing judgment (self relation).
\end{revviiib}


\et{the last line of Fig2 should present *semantic* typing (with $\vDash$), then your type soundness result is $... \vdash e : G \implies ...\vDash e : G $}


\mt{HERE}
\mt{I see some options:
\begin{enumerate}
  \item (1) Soudness, leaving typing abstract, (2) typing and then (3) runtime
  \item (1) typing (2) soundness (3) runtime
  \item (1) typing (2) runtime (1) soundness.
  \item (1) runtime, abstract operators, (1) typing, (3) soundness (4) instantiation of abstract operators such as transitivity.
\end{enumerate}
What about the elaboration?
}

\begin{revviiib}
\mt{Move to section about extending this to GSOUL.} Due to the presence of recursive types in \lang, the full definition of the logical relation for \lang (found in the supplementary material) uses step indexing to ensure well-foundedness, albeit in a standard manner.
\end{revviiib}

The semantic model of

% % Note that the \reviv{homogeneous} type-and-effect syntax allows us to encode latent effects \reviv{without having to annotate arrows or other type constructors}.
% The used type-and-effect syntax naturally captures the idea of latent effects.\da{cite Toro et al. on latent effects?}
% \reviv{For example, the type-and-effect of an expression that reduces to a function has the form $\itype{(\itype{\gty[1]}{\gsenv[1]} \rightarrow \itype{\gty[2]}{\gsenv[2]})}{\gsenv}$, where $\gsenv[1]$ is the expected effect of the argument, $\gsenv[2]$ is called the \textit{latent effect} of the produced function and $\gsenv$ is the effect of evaluating the expression.
% As usual in type-and-effect systems, a latent effect ensures that the effect of the body of the produced function is accounted for upon each function application.}




\begin{figure*}[t]
  \raggedright
  \begin{small}

  \textbf{Well-typed gradual expressions} \hfill
  \boxed{\sttyping{e}{\cgty}} \\
  \begin{mathpar}
    \inferrule*[lab=\Grefr{const}]{ }{
      \sttyping{c}{\itype{\mathit{ty}(c)}{\emptysenv}}
    }

    \inferrule*[lab=\Grefr{op}]{
      \overline{\sttyping{e_i}{\cgty[i]}} \\
      \bopFuncName[\bop](\overline{\cgty[i]}) = \cgty
    }{
      \sttyping{
        \bop \overline{e_i}
      }{
        \cgty
      }
    }

    \inferrule*[lab=\Grefr{$\Lambda$}]{
      \sttyping[\tenv][\svenv, \r]{e}{\cgty}
    }{
      \sttyping{\polyS[\r]. e}{\itype{(\polyST[\r].\cgty)}{\emptysenv}}
    }

    \inferrule*[lab=\Grefr{app}]{
      \sttyping{e_1}{\cgty[1]} \\
      \sttyping{e_2}{\cgty[2]} \\
      \cgty[2] \ccsub \domm(\cgty[1])
    }{
      \sttyping{
        e_1 \app e_2
      }{
        \codd(\cgty[1])
      }
    }

    \inferrule*[lab=\Grefr{inst}]{
      \sttyping{e}{\cgty} \\
      \typewfs{\gsenv}
    }{
      \sttyping{e \appS{\gsenv}}{\instt(\cgty, \gsenv)}
    }

    \inferrule*[lab=\Grefr{ascr},width=4cm]{
      \sttyping{e}{\cgty} \\
      \cgty \ccsub \cgtyp \\
      \typewfs{\cgtyp}
    }{
      \sttyping{e \ascr{\cgtyp}}{\cgtyp}
    }
  \end{mathpar}

  \begin{mathpar}
  	\itype{\gty}{\gsenv} \effOp{\textsf{+}} \gsenvp = \teff{\gty}{\gsenv + \gsenvp} \and
    \domm(\itype{(\cgty[1] \rightarrow \cgty[2])}{\gsenv}) = \cgty[1] \and
    \codd(\itype{(\cgty[1] \rightarrow \cgty[2])}{\gsenv}) = \cgty[2] \effOp{+} \gsenv
    \and
    \instt(\itype{\polyS.\cgty[2]}{\gsenv}, \gsenv[1]) = \substv{\gsenv[1]}{\SG{\r}}{\cgty[2]} \effOp{+} \gsenv
    \and
    \bopFuncName[+](\itype{\rtype}{\gsenv[1]}, \itype{\rtype}{\gsenv[2]}) = \itype{\rtype}{\gsenv[1] + \gsenv[2]} \and
    \bopFuncName[*](\itype{\rtype}{\gsenv[1]}, \itype{\rtype}{\gsenv[2]}) = \itype{\rtype}{\infty(\gsenv[1] + \gsenv[2])} \and
    \bopFuncName[\leq](\itype{\rtype}{\gsenv[1]}, \itype{\rtype}{\gsenv[2]}) = \itype{\btype}{\infty(\gsenv[1] + \gsenv[2])}
  \end{mathpar}
  \end{small}
  \caption{Type system of \GSoulCore (excerpt)}
  \label{fig:lifted-type-sytem}
\end{figure*}

% \begin{figure}[t]
%   \raggedright

%   \begin{small}

%   \textbf{Precision of sensitivity effects} \hfill
%   \boxed{\gsenv \gprec \gsenv} \\
%   \begin{mathpar}
%     \inferrule*{ }{
%       \emptysenv \gprec \emptysenv
%     }

%     \inferrule*{
%       \gsenv[1] \gprec \gsenv[2]\\
%       \gsens[1] \gprec \gsens[2]
%     }{
%       \gsenv[1] + \gsens[1] x \gprec
%       \gsenv[2] + \gsens[2] x
%     }
%   \end{mathpar}

%   \textbf{Precision of \tyclsPlur} \hfill
%   \boxed{\gty \gprec \gty} \\
%   \begin{mathpar}
%     \inferrule{
%       \gty \in \set{\rtype, \btype}
%     }{
%       \gty \gprec \gty
%     }

%     \inferrule{
%       \cgty[1] \gprec \cgtyp[1]\\
%       \cgty[2] \gprec \cgtyp[2]
%     }{
%       \cgty[1] \rightarrow \cgty[2] \gprec
%       \cgtyp[1] \rightarrow \cgtyp[2]
%     }

%     \inferrule{
%       \cgty \gprec \cgtyp\\
%     }{
%       \polyST. \cgty \gprec
%       \polyST. \cgtyp
%     }
%   \end{mathpar}

%   \textbf{Precision of \typeclsPlur} \hfill
%   \boxed{\cgty \gprec \cgty} \\
%   \begin{mathpar}
%     \inferrule*{
%       \gty[1] \gprec \gty[2]\\
%       \gsenv[1] \gprec \gsenv[2]
%     }{
%       \itype{\gty[1]}{\gsenv[1]} \gprec \itype{\gty[2]}{\gsenv[2]}
%     }
%   \end{mathpar}
%   \end{small}

%   \caption{Precision of Gradual Sensitivity Types}
%   \label{fig:type-prec}
% \end{figure}

\subsection{A Gradual Sensitivity Type System}

The typing rules for \GSoulCore are presented in Figure \ref{fig:lifted-type-sytem}.
\rev{
  The judgment $\sttyping{e}{\cgty}$ establishes that expression $e$ has type-and-effect $\cgty$ under \typeclsSing{} environment $\tenv$ and resource set $\svenv$, where $\tenv$ is a mapping from variables to \typeclsPlur{} and $\svenv$ is a set of the resource variables in scope.
}
\revviii{Since the type-and-effect $\cgty$ contains sensitivity information, the type system is designed to capture the sensitivity of $e$ with respect to the resources contained in $\svenv$.}
Typing rules are standard except for the handling of sensitivity effects.
\Grefr{const} and \Grefr{$\Lambda$} report no effect, $\emptysenv$, as they are introduction forms and thus no resource variables are being used.
\reviv{Constants $c$ are typed using the auxiliary function $ty(c)$, and primitive n-ary operations $\bop$ are given meaning by the function $\bopFuncName$,  which handles the treatment of sensitivity information. }
The effect of addition $\bopFuncName[+]$ is computed by adding the effect of each sub-expression.
The addition \revii{of sensitivity effects} is defined by adding the sensitivities of each variable, \ie~$\SG{(\gsenv[1] + \gsens[1]\r) + (\gsenv[2] + \gsens[2]\r)} = \SG{(\gsenv[1] + \gsenv[2]) + (\gsens[1] + \gsens[2])\r}$.
Addition ($\SG{+}$), multiplication ($\SG{*}$), join ($\SG{\sjoin}$) and meet ($\SG{\smeet}$) of gradual sensitivities is defined bound-wise, \ie~for addition: $\SG{\sensint{\sens[1], \sens[2]} + \sensint{\sens[3], \sens[4]}} = \SG{\sensint{\sens[1] + \sens[3], \sens[2] + \sens[4]}}$.
The join and meet of two static sensitivities is the maximum and minimum of both, respectively.
The effect of a comparison $\bopFuncName[\leq]$ scales to infinite the addition of the sensitivity effects of each sub-expression because a small variation on one of the sub-expressions could change the result from $\true$ to $\false$, which are considered $\infty$ apart \cite{reedAl:icfp2010}.
The scaling of effects is defined naturally: $\SG{\gsens(\gsenv + \gsensp \r)} = \SG{\gsens\gsenv + (\gsens * \gsensp)\r}$.
Lastly, the effect of a multiplication $\bopFuncName[*]$ is computed scaling the addition of the sensitivity effects of each sub-expression by $\infty$.
The choice of syntax for types ensures that latent effects are naturally captured by introduction rules, while being standard.
As expected, rule \Grefr{$\Lambda$} is the only one that extends the resource variables set $\svenv$.

For \Grefr{app} we follow the presentation of \citet{garciaAl:popl2016}, using partial meta-functions $\domm$ and $\codd$ to extract the domain and codomain of a function \typeclsSing.
% However, we have to adapt these functions to work on a type-and-effect system.
The $\codd$ function reports not only the effect of reducing the expression to a value, $\gsenv$, but also the latent effect of the function, contained in $\cgty[2]$, and the effect of reducing the expression to a function.
\reviii{We do this by leveraging the $\effOp{+}$ operator that sums a given effect to a type-and-effect.}
This way, we account for the latent effect of the body at application time.
More generally, we define $\itype{\gty}{\gsenv} \effOp{\mathsf{op}} \gsenvp = \itype{\gty}{\gsenv \mathbin{\SG{\mathsf{op}}} \gsenvp}$, where $\SG{\mathsf{op}}$ denotes a binary operation between two sensitivity effects.

\rev{
  Rule \Grefr{inst} removes a resource from scope by instantiating it with a sensitivity effect $\gsenv$.
  We use a meta-function $\instt$ that works in a similar fashion to $\codd$, but also performs a substitution of the resource $\r$ with the sensitivity effect passed as argument.
  \hide{Well-formedness of sensitivity effects, types and type-and-effects with respect to a resource variables set is defined to ensure that the use of variables are well-scoped.}
}
A sensitivity effect substitution, $\substv{\gsenv[1]}{\r}{\gsenv}$, replaces all occurrences of $\r$ in $\gsenv$ by $\gsenv[1]$.
For example, $\substv{\SG{2\r[2] + \r[3]}}{\r[1]}{\SG{(3\r[1] + \unknown\r[2])}} = \SG{3(2\r[2] + \r[3]) + \unknown\r[2]} = \SG{(6 + \unknown)\r[2] + 3\r[3]} = \SG{\sensint{6,\infty}\r[2] + 3\r[3]}$.
The judgment $\typewfs{\cgty}$ (and $\typewfs{\gsenv}$) ensures that the \typeclsSing{} $\cgty$ (and $\gsenv$, respectively) only contains resources contained in $\svenv$ and can be found in the supplementary material.

As previously mentioned, \GSoulCore relies on a relaxed notion of subtyping: consistent subtyping.
Instead of checking for exact subtyping, consistent subtyping checks if it is \emph{plausible} that a type is a subtype of another.
We start by defining consistent subtyping for gradual sensitivities:

\begin{definition}[Consistent Sensitivity Subtyping]
  \label{def:consistent-sens-subtyping}
  $\sensint{\sens[1], \sens[2]} \ccleq \sensint{\sens[3], \sens[4]}$ if and only if $\sens[1] \leq \sens[4]$.
\end{definition}

Intuitively, a gradual sensitivity $\gsens[1]$ is optimistically less or equal to another, $\gsens[2]$, if there \emph{exists} a sensitivity within $\gsens[1]$ that is less or equal to another one within $\gsens[2]$.
This is easily checkable by comparing the lower bound of $\gsens[1]$ with the upper bound of $\gsens[2]$.
Consistent subtyping for effects, \tyclsPlur and \typeclsPlur, denoted by $\ccsub$, is defined naturally from Definition~\ref{def:consistent-sens-subtyping} and can be found in the supplementary material.

\da{revA: \quot{I cannot understand anything here}}
% \paragraph{Plausibility in the Type System}
The type system of \GSoulCore optimistically accepts judgments that \emph{may} hold during runtime.
For instance, consider the type derivation: $\sttyping[x: \teff{\rtype}{\r}][\r]{(x + x) \ascr{\teff{\rtype}{\unknown \r}} \ascr{\teff{\rtype}{\r}}}{\teff{\rtype}{\r}}$.
% \begin{small}
% \begin{mathpar}
%   \inferrule*[lab=\Grefr{ascr}]{
%     \inferrule*[lab=\Grefr{ascr}]{
%       \sttyping{2x}{\teff{\rtype}{2\r}}\\
%       \teff{\rtype}{2\r} \ccsub \teff{\rtype}{\unknown \r}
%     }{
%       \sttyping{2x \ascr{\teff{\rtype}{\unknown \r}}}{\teff{\rtype}{\unknown \r}}
%     }\\
%     \teff{\rtype}{\unknown \r} \ccsub \teff{\rtype}{\r}
%   }{
%     \sttyping{
%       (2x \ascr{\teff{\rtype}{\unknown \r}}) \ascr{\teff{\rtype}{\r}}
%     }{\teff{\rtype}{\r}}
%   }
% \end{mathpar}
% \end{small}
% open expression $e = (x + x) \ascr{\teff{\rtype}{\unknown \r}} \ascr{\teff{\rtype}{\r}}$, a resource set $\svenv = \r$ and a type environment $\tenv = x: \teff{\rtype}{\r}$.
Given that both $\teff{\rtype}{2\r} \ccsub \teff{\rtype}{\unknown \r}$ and $\teff{\rtype}{\unknown \r} \ccsub \teff{\rtype}{\r}$ hold, such derivation can be easily constructed using the rule \Grefr{ascr} twice.
This is because, given the removal of precision through the use of $\unknown$, for the typechecker it is \textit{plausible} that they might hold at runtime.
\et{step back: what's the point of the paragraph? what do you want to say/illustrate? why here?}
\et{if you keep the example then start from the example program, not from the typing derivation of an open term}

\begin{comment}
The type derivation of $e$ follows as:

\begin{small}
\begin{mathpar}
  \inferrule*[left=\Grefr{ascr}]{
    \inferrule*[left=\Grefr{ascr}]{
      \sttyping{2x}{\teff{\rtype}{2\r}}\\
      \teff{\rtype}{2\r} \ccsub \teff{\rtype}{\unknown \r}
    }{
      \sttyping{2x \ascr{\teff{\rtype}{\unknown \r}}}{\teff{\rtype}{\unknown \r}}
    }\\
    \teff{\rtype}{\unknown \r} \ccsub \teff{\rtype}{\r}
  }{
    \sttyping{
      (2x \ascr{\teff{\rtype}{\unknown \r}}) \ascr{\teff{\rtype}{\r}}
    }{\teff{\rtype}{\r}}
  }
\end{mathpar}
\end{small}

Notice how both subtyping judgments, $\teff{\rtype}{\unknown \r} \ccsub \teff{\rtype}{\r}$ and $\teff{\rtype}{2\r} \ccsub \teff{\rtype}{\unknown \r}$, hold.
This is because, given the removal of precision through the use of $\unknown$, for the typechecker it is \textit{plausible} that they might hold at runtime.
\end{comment}

\begin{revviiib}
\subsection{A Preview of the Runtime Semantics}
\label{sec:dynamic-semantics-preview}

In order to account for optimism during typechecking, gradual runtime semantics perform runtime checks, raising an error whenever a static typing assumption is about to be violated. In general, the runtime semantics of gradual languages are given by a translation to cast calculi, where casts are inserted to perform such checks~\cite{siekTaha:sfp2006}.
\GSoulCore is no exception: evaluating a \GSoulCore expression is a process that first translates the expression to a cast calculus, called \GSoulEvCore, and then reduces this elaborated expression to a value, or halts with an error if cast fails.
We write $\lceil e \rceil$ to denote the translation of a closed \GSoulCore expression $e$, i.e an expression with no free variables, to \GSoulEvCore.
%
We write $e \mapsto^{*} v$ to denote that a \GSoulEvCore expression $e$ reduces in several steps to a value $v$.
Furthermore, we write $e \Downarrow v$ to denote that a \GSoulCore expression $e$ evaluates to a value $v$, \ie~$e \Downarrow v$ if and only if $\lceil e \rceil \mapsto^{*} v$.
A detailed explanation of the runtime semantics of \GSoulEvCore is provided in \S\ref{sec:dynamic-semantics}, but for now, we provide a brief overview sufficient to understand the gradual sensitivity semantics of \GSoulCore.


Crucially, any \GSoulEvCore value (\eg~integers, booleans, lambdas) is enriched with collected runtime information about the sensitivity effects of the expression that produced it. Given a value $v$, we use the meta-function $\getVal$ to access the underlying value and $\getEff$ to retrieve the (runtime) sensitivity effect.
For instance, given two resources $r_1 = 10$ and $r_2 = 20$, we have
$2*r1 + r2 \Downarrow v$, with $\getVal(v) = 40$ and $\getEff(v) = 2r_1 + r_2$. \da{Fix this}

In general, if $v$ has type $\itype{\gty}{\gsenv}$ and $\gsenvp = \getEff(v)$, it means that the monitored sensitivity effect of $v$ is $\gsenvp$, which corresponds to a more precise version of $\gsenv$.
Precision in the context of gradual sensitivities corresponds to interval inclusion.
Formally, $\sensint{\sens[1], \sens[2]}$ is more precise than $\sensint{\sens[3], \sens[4]}$, written $\sensint{\sens[1], \sens[2]} \gprec \sensint{\sens[3], \sens[4]}$, if and only if $\sens[1] \geq \sens[3]$ and $\sens[2] \leq \sens[4]$.
Precision for gradual sensitivity effects, \tyclsPlur and \typeclsPlur is naturally defined from gradual sensitivities precision, \eg~$\SG{\sensint{2, 8}\r[1] + \sensint{2,\infty}\r[2]} \gprec \SG{\sensint{0, 10}\r[1] + ?\r[2]}$ because $\sensint{2, 8} \gprec \sensint{0, 10}$ and $\sensint{2, \infty} \gprec \sensint{0, \infty}$.
The full definitions for precision can be found in the supplementary material.\et{should be in the corresponding section within the paper (that's too crucial to leave out)}
\end{revviiib}


==> sections/implementation.tex <==
%!TEX root = ../main.tex
\section{Implementation}
\label{sec:implementation}

\lang is implemented as a prototype written in Typescript. The toolchain can be found at \href{https://darquezt.github.io/gsoul-lang/}{https://darquezt.github.io/gsoul-lang/}.

The interpreter is not meant to be an efficient implementation, but to serve as a reference and provide a playground to run interesting programs, and test the benefits and limitations of gradual sensitivity typing.

The implementation is able to both typecheck and reduce a program.
Running a program consists of three main phases: parsing and desugaring source code, elaborating (while typechecking) to evidence-augmented terms, and reducing the program.
The implementation of the elaboration and typechecking follows Figure~\ref{fig:intrinsic-elaboration}.
Reduction is implemented as a CEK machine~\cite{felleisen:fdpc1986}, closely following the reduction rules for \lambdaGSensEv{}.
The abstraction and concretization functions are not used directly: all type predicates, functions, and operators are implemented using their equivalent algorithmic characterizations.

Besides the already presented features of \lang, the implementation also supports let and (recursive) function declarations.
Low-level features of the language, such as big lambdas for resource polymorphism, are not intended to be used by end-users.
Instead, we use them for building ergonomic features, such as the \lstinline[language=gsoul]|res| modifier.
Programmers can declare resources using \lstinline[language=gsoul]|let res|, which besides binding a variable, it also creates a resource with the same name at types level.

\begin{small}
\begin{lstlisting}[language=gsoul,numbers=none]
let r = 1;          // normal variable; type: Number
let res b = false;  // resource variable; type: Boolean[b]
\end{lstlisting}
\end{small}

Alternatively to using the \lstinline|def _[r](...)| syntax, function parameters can be declared as polymorphic resources, using the \lstinline[language=gsoul]|res| modifier.

\begin{small}
\begin{lstlisting}[language=gsoul,numbers=none]
def double(res x: Number): Number[2x] = x + x;
\end{lstlisting}
\end{small}

Finally, we augment the language with a \lstinline|List|, \lstinline|Set|, and \lstinline|Map| types, and a few primitives for manipulating them, as well as algebraic datatypes (encoded using recursive types) and type polymorphism.\footnote{
  Notice that lists can already be encoded using datatypes types (which can be encoded from recursive types). However, we introduce them as a primitive type for improving the ergonomics of the language.
}
We expect to further extend the language with more features, which hopefully will lead to interesting use cases and challenges for gradual sensitivity typing.
% The following program is the \lang analogous to the one presented by \citet{reedAl:icfp2010} for \Fuzz, which computes the histogram of a list of numbers.

% \begin{small}
% \begin{lstlisting}[language=gsoul,numbers=none]
% def histAux(c: Number, res db: Set<Number>): List<Set<Number>[db]> {
%   if (c >= 101) List(db)
%   else {
%     let bin, next = db.split(fn (x: Number) => c >= x);
%     bin :: histAux(c + 10, next);
%   }
% }

% let hist = fn (res db: Set<Number>): List<Number[db]> => histAux(0, db).map(
%   fn (res bin: Set<Number>) => bin.size()
% );
% \end{lstlisting}
% \end{small}


==> sections/minisax.tex <==
%!TEX root = ../main.tex
\section{\SoulCore: A Core Static Sensitivity Typing}
\label{sec:static-lang}

In this section we present \SoulCore, a \reviv{core} language with static sensitivity typing.
We use {\color{StoreGreen} green} for sensitivity related variables, and {\color{EqBlue}blue} for the rest of the math notation.
\rev{
  The semantics of the language are initially based on \Sax~\cite{toroAl:toplas2023} and its latent type-and-effect discipline, here extended with ascriptions and explicit sensitivity polymorphism.
}

\begin{figure}[tp]
  \begin{small}
  \centering

  \begin{align*}
    c \in \rtype \cup \btype, \quad
    x \in \VarClass, \quad
    e \in \ExprClass, \quad
    \sens \in \SensClass \triangleq \rtype^{\geq 0} \cup \{ \infty \}, \quad
    \r \in \ResClass, \quad
    \senv \in \SenvClass, \quad
    \sty \in \TyClass, \quad
    \cty \in \TypeClass
  \end{align*}
  \begin{align*}
    e ::= {}&
      c \mid \bop \overline{e} \mid
      x \mid \lambda (x:\cty). e \mid e \app e
      \mid \polyS[\r]. e \mid
      e \appS{\senv} \mid e \ascr{\cty}
      & \syntaxLabel{expressions}\\
    %
    \senv ::= {}& \SG{\sens \r + \dots + \sens \r}
      & \syntaxLabel{sensitivity effects}\\
    %
    \sty ::= {}&
      \rtype \mid
      \btype \mid
      \cty \rightarrow \cty \mid
      \polyST[\r]. \cty
      & \syntaxLabel{types}\\
    %
    \cty ::= {}&
      \itype{\sty}{\senv}
      & \syntaxLabel{type-and-effects}
  \end{align*}

  \textbf{Well-typed Expressions} \hfill \boxed{\ssttyping{e}{\cty}}
  \begin{mathpar}
  \inferrule*[lab=\Trefr{const}]{ }{
    \ssttyping{c}{\itype{\mathit{ty}(c)}{\emptysenv}}
  }

  \inferrule*[lab=\Trefr{op}]{
    \overline{\ssttyping{e_i}{\cty[i]}} \\
    \bopFuncName[\bop](\overline{\cty[i]}) = \cty
  }{
    \ssttyping{
      \bop \overline{e_i}
    }{
      \cty
    }
  }

  \inferrule*[lab=\Trefr{var}]{ }{
    \ssttyping{x}{\Gamma(x)}
  }

  \inferrule*[lab=\Trefr{lam}]{
    \ssttyping[\tenv, x:\cty[1]]{e}{\cty[2]} \\
    \typewfs{\cty[1]}
  }{
    \ssttyping{
      \lambda (x:\cty[1]).e
    }{
      \itype{(\cty[1] \rightarrow \cty[2])}{\emptysenv}
    }
  }

  \inferrule*[lab=\Trefr{$\Lambda$}]{
    \ssttyping[\tenv][\svenv, \SG{\r}]{e}{\cty}
  }{
    \ssttyping{\polyS. e}{\itype{(\polyST.\cty)}{\emptysenv}}
  }

  \inferrule*[lab=\Trefr{inst}]{
    \ssttyping{e}{\cty} \\
    \typewfs{\senv}
  }{
    \ssttyping{e \appS{\senv}}{\instt(\cty, \senv)}
  }

  \inferrule*[lab=\Trefr{app}]{
    \ssttyping{e_1}{\cty[1]} \\
    \ssttyping{e_2}{\cty[2]} \\
    \cty[2] \subty \domm(\cty[1])
  }{
    \ssttyping{
      e_1 \app e_2
    }{
      \codd(\cty[1])
    }
  }

  \inferrule*[lab=\Trefr{ascr}]{
    \ssttyping{e}{\cty} \\
    \cty \subty \ctyp \\
    \typewfs{\ctyp}
  }{
    \ssttyping{e \ascr{\ctyp}}{\ctyp}
  }


  \end{mathpar}

  \begin{mathpar}
  	\itype{\sty}{\senv} \effOp{\textsf{+}} \senvp = \teff{\sty}{\senv + \senvp} \and
    \domm(\itype{\cty[1] \rightarrow \cty[2]}{\senv}) = \cty[1] \and
    \codd(\itype{\cty[1] \rightarrow \cty[2]}{\senv}) = \cty[2] \effOp{+} \senv
    \\
    \instt(\itype{\polyS.\cty[2]}{\senv}, \senv[1]) = \substv{\senv[1]}{\SG{\r}}{\cty[2]} \effOp{+} \senv
    \and
    \bopFuncName[+](\itype{\rtype}{\senv[1]}, \itype{\rtype}{\senv[2]}) = \itype{\rtype}{\senv[1] + \senv[2]} \and
    \bopFuncName[*](\itype{\rtype}{\senv[1]}, \itype{\rtype}{\senv[2]}) = \itype{\rtype}{\infty(\senv[1] + \senv[2])} \and
    \bopFuncName[\leq](\itype{\rtype}{\senv[1]}, \itype{\rtype}{\senv[2]}) = \itype{\btype}{\infty(\senv[1] + \senv[2])}
  \end{mathpar}

  \textbf{Subtyping} \hfill
  \boxed{\senv \subty \senv}

  \begin{align*}
      \senv[1] \subty \senv[2] &\Leftrightarrow \forall \r \in \dom(\senv[1]) \cup \dom(\senv[2]). \senv[1](\r) \leq \senv[2](\r)
  \end{align*}

  \begin{minipage}{0.6\textwidth}
    \hfill \boxed{\sty \subty \sty}

    \begin{mathpar}
      \inferrule*[lab=\Trefr{sub-base}]{
        \sty \in \set{\rtype, \btype}
      }{
        \sty \subty \sty
      }

      \inferrule*[lab=\Trefr{sub-arrow}]{
        \cty[21] \subty \cty[11] \\
        \cty[12] \subty \cty[22]
      }{
        \cty[11] \rightarrow \cty[12] \subty
        \cty[21] \rightarrow \cty[22]
      }

      \inferrule*[lab=\Trefr{sub-sabs}]{
        \cty[1] \subty \cty[2]
      }{
        \polyST . \cty[1] \subty
        \polyST . \cty[2]
      }
    \end{mathpar}
  \end{minipage}
  \begin{minipage}{0.39\textwidth}
    \hfill \boxed{\cty \subty \cty}

    \begin{mathpar}
      \inferrule*[lab=\Trefr{sub-teff}]{
        \sty[1] \subty \sty[2] \\
        \senv[1] \subty \senv[2]
      }{
        \itype{\sty[1]}{\senv[1]} \subty
        \itype{\sty[2]}{\senv[2]}
      }
    \end{mathpar}
  \end{minipage}

  \end{small}
  \caption{\SoulCore: Syntax and Type System.}
  \label{fig:static-syntax}
\end{figure}

% \begin{figure}[t]

%   \begin{small}

%   \textbf{Well sensitivity formedness of sensitivity environments}\hfill
%   \boxed{\typewfs{\senv}} \\
%   \begin{mathpar}
%     \inferrule*{ }{
%       \typewfs{\emptysenv}
%     }

%     \inferrule*{
%       \typewfs{\senv}\\
%       \r \in \svenv
%     }{
%       \typewfs{\senv + \sens \r}
%     }
%   \end{mathpar}

%   \textbf{Well sensitivity formedness of types} \hfill
%   \boxed{\typewfs{\sty}}\\
%   \begin{mathpar}
%     \inferrule*{
%       \sty \in \set{\rtype, \btype}
%     }{
%       \typewfs{\sty}
%     }

%     \inferrule*{
%       \typewfs{\cty[1]}\\
%       \typewfs{\cty[2]}
%     }{
%       \typewfs{\cty[1] \rightarrow \cty[2]}
%     }

%     \inferrule*{
%       \typewfs[\svenv, \r]{\cty}
%     }{
%       \typewfs{\polyST[\r] . \cty}
%     }
%   \end{mathpar}

%   \textbf{Well sensitivity formedness of type-and-effects} \hfill
%   \boxed{\typewfs{\cty}}\\
%   \begin{mathpar}
%     \inferrule*{
%       \typewfs{\sty}\\
%       \typewfs{\senv}
%     }{
%       \typewfs{\itype{\sty}{\senv}}
%     }
%   \end{mathpar}
%   \end{small}

%   \caption{Type Well-formedness}
%   \label{fig:static-wf}
% \end{figure}

% \begin{figure}
%   \begin{align*}
%     \rsubst{\sty}{\recvar}\recvarp &= \itype{\sty}{\emptysenv}  \quad \text{if} ~ \recvar = \recvarp\\
%     \rsubst{\sty}{\recvar}\recvarp &= \recvarp                  \quad \text{if} ~ \recvar \neq \recvarp\\
%   \end{align*}
% \end{figure}

\paragraph{Syntax}
The \reviv{syntax} of \SoulCore are presented in Figure~\ref{fig:static-syntax}. Expressions $e$ include \reviv{constants, primitive operations}, variables, lambda expressions, applications, \rev{sensitivity abstractions, sensitivity effect applications,} and ascriptions.

A \tyclsSing{} $\sty$ can be the real number type $\rtype$, \reviv{the boolean type $\btype$,} a function type $\cty \rightarrow \cty$, or a \reviv{resource} quantification $\polyST. \cty$. A type-and-effect
$\cty$ is a tuple $\itype{\sty}{\senv}$ associating a type $\sty$ and a sensitivity effect $\senv$, which is a mapping between resource variables $\SG{\r}$ and sensitivities $\sens$.
\reviv{
  Across the paper, we use meta-variables $x, y, z$ (written in {\color{EqBlue}blue}) for lambda-bound variables and $\r$ (written in \SG{green}) for resource variables.
}
A sensitivity $\sens$ is a positive real number or infinity, where $\sinfty \cdot \SG{0} = \SG{0} \cdot \sinfty = \SG{0}$ and $\sens \cdot \sinfty = \sinfty \cdot \sens = \sinfty$ if $\sens > \SG{0}$.
For simplicity we write effects as first-order polynomials, \eg~$\senv = \SG{\r[1] + 3\r[2]}$ is a sensitivity effect where $\senv(\SG{\r[1]}) = \SG{1}$, $\senv(\SG{\r[2]}) = \SG{3}$\revii{, and $\senv(\r) = \SG{0}$ for any other resource $\r$ in scope}.
%Also, whenever a sensitivity variable in scope is not mentioned in the environment, then its sensitivity is assumed to be zero, \ie~$\senv(z) = \SG{0}$ when $z \not\in \dom(\svenv)$.

Note that the \reviv{homogeneous} type-and-effect syntax allows us to encode latent effects in a similar fashion to \Sax, \reviv{without having to annotate arrows or other type constructors}.
\reviv{For example, the type-and-effect of an expression that reduces to a function has the form $\itype{(\itype{\sty[1]}{\senv[1]} \rightarrow \itype{\sty[2]}{\senv[2]})}{\senv}$, where $\senv[1]$ is the expected effect of the argument, $\senv[2]$ is called the \textit{latent effect} of the produced function and $\senv$ is the effect of evaluating the expression.
As usual in type-and-effect systems, a latent effect ensures that the effect of the body of the produced function is accounted for upon each function application.}

\paragraph{Typechecking sensitive expressions}
\rev{
  The typing judgment $\ssttyping{e}{\cty}$ establishes that expression $e$ has type-and-effect $\cty$ under \typeclsSing{} environment $\tenv$ and resource set $\svenv$, where $\tenv$ is a mapping from variables to \typeclsSing{} and $\svenv$ is a set of the resource variables in scope.
}
Typing rules are standard except for the handling of sensitivity effects.
\Trefr{const}, \Trefr{lam} and \Trefr{$\Lambda$} report no effect, $\emptysenv$, as they are introduction forms and thus no resource variables are being used.
\reviv{Constants $c$ are typed using the auxiliary function $ty(c)$, and primitive n-ary operations $\bop$ are given meaning by the function $\bopFuncName$,  which handles the treatment of sensitivity information. }
The effect of addition $\bopFuncName[+]$ is computed by adding the effect of each sub-expression.
The addition \revii{of sensitivity effects} is defined by adding the sensitivities of each variable, \ie~$\SG{(\senv[1] + \sens[1]\r) + (\senv[2] + \sens[2]\r)} = \SG{(\senv[1] + \senv[2]) + (\sens[1] + \sens[2])\r}$.
The effect of a comparison $\bopFuncName[\leq]$ scales to infinite the addition of the sensitivity effects of each sub-expression because a small variation on one of the sub-expression could change the result from $\true$ to $\false$, which are considered $\infty$ apart \cite{reedAl:icfp2010}.
The scaling of effects is defined naturally: $\SG{\sens(\senv + \sensp \r)} = \SG{\sens\senv + (\sens \cdot \sensp)\r}$.
Lastly, the effect of a multiplication $\bopFuncName[*]$ is computed scaling the addition of the sensitivity effects of each sub-expression by $\infty$.
The choice of \revii{syntax for }types \revii{ensure} that latent effects are naturally captured by rules \Trefr{lam} and \Trefr{$\Lambda$}, while being standard.
\reviv{
  In contrast to previous work~\cite{reedAl:icfp2010,nearAl:oopsla2010,toroAl:toplas2023}, resources are explicitly introduced using resource abstraction $\polyS[\r]. e$, where the resource variable $\r$ is bound in the body $e$.
}
As expected, rule \Trefr{$\Lambda$} is the only one that extends the resource variables set $\svenv$, and is otherwise analogous to \Trefr{lam}.
\revii{
  The judgment $\typewfs{\cty}$ ensures that the \typeclsSing{} $\cty$ only contains sensitive variables contained in $\svenv$ and can be found in the supplementary material.
}

For \Trefr{app} we follow the approach of \citet{garciaAl:popl2016}:
in order to anticipate the gradualization, we formulate the rule using partial meta-functions $\domm$ and $\codd$ to extract the domain and codomain of a function \typeclsSing{}, respectively.
However, we have to adapt the functions to work on a type-and-effect system.
The definition of $\domm$ is analogous to the original definition, but the $\codd$ function reports not only the effect of reducing the expression to a value, $\senv$, but also the latent effect of the function, contained in $\cgty[2]$, and the effect of reducing the expression to a function.
\reviii{We do this by leveraging the $\effOp{+}$ operator that sums a given effect to a type-and-effect.}
This way, we account for the latent effect of the body at application time.

\rev{
  Rule \Trefr{inst} removes a sensitive variable from scope by instantiating it with a well-formed sensitivity effect $\senv$.
  We use a meta-function $\instt$ that works in a similar fashion to $\codd$, but also performs a substitution of the resource $\r$ with the sensitivity effect passed as argument.
  Well-formedness of sensitivity effects, types and type-and-effects with respect to a resource variables set is defined to ensure that the use of variables are well-scoped.
}
A sensitivity effect substitution, $\substv{\senv[1]}{\r}{\senv}$, replaces all occurrences of $\r$ in $\senv$ by $\senv[1]$.
For example, $\substv{\SG{2\r[2] + \r[3]}}{\r[1]}{\SG{(3\r[1] + \r[2])}} = \SG{3(2\r[2] + \r[3]) + \r[2]} = \SG{7\r[2] + 3\r[3]}$.

\begin{figure}[t]

  \raggedright
  \begin{small}
  % \begin{align*}
  %   v \in \ValClass
  % \end{align*}
  \begin{align*}
    e ::= {}&
      \dots \mid
      \sctx{\r}{\senv}(e)
      & \syntaxLabel{expressions}\\
    %
    v ::= {}&
      c \mid
      \lambda (x:\cty).e \mid
      \polyS .e
      & \syntaxLabel{values}\\
    %
    \Ectx ::= {}&
      \emptycontext \mid
      \bop \overline{v_i}\, \Ectx\, \overline{e_i} \mid
      \Ectx \app e \mid
      v \app \Ectx \mid
      \Ectx \appS{\senv} \mid
      \sctx{\r}{\senv}(\Ectx) \mid
      \Ectx \ascr{\cty}
      & \syntaxLabel{evaluation contexts}
  \end{align*}

  \textbf{Notions of reduction} \hfill
  \boxed{\phantom{|}e \longrightarrow e\phantom{|}}

  \begin{minipage}{0.4\textwidth}
    \begin{align*}
      \Trefr{r-plus} & &
      \bop \overline{c_i} &
      \longrightarrow
      \llbracket \bop \rrbracket\, \overline{c_i}\\
      %
      \Trefr{r-app} & &
      (\lambda (x:\cty).e) \app v
      & \xlongrightarrow{}
      [v/x]e\\
      %
      \Trefr{r-inst} & &
      (\polyS[\r].e )\appS{\senv}
      & \xlongrightarrow{}
      \sctx{\r}{\senv}(e)
    \end{align*}
  \end{minipage}
  \begin{minipage}{0.5\textwidth}
    \begin{align*}
      %
      \Trefr{r-sctx} & &
      \sctx{\r}{\senv}(v)
      & \xlongrightarrow{}
      \substv{\senv}{\SG{\r}}{v}\\
      %
      \Trefr{r-ascr} & &
      v \ascr{\cty}
      & \xlongrightarrow{}
      v
    \end{align*}
  \end{minipage}
  \end{small}
  \caption{\SoulCore: Dynamic semantics (excerpt)}
  \label{fig:static-dynamics}
\end{figure}

\paragraph{Dynamic Semantics} The dynamic semantics of \SoulCore are call-by-value, formalized using evaluation contexts.
The extended syntax and an excerpt of the reduction rules are presented in Figure~\ref{fig:static-dynamics}.
Values can be \reviv{constants, lambdas and resource abstractions}.
\reviv{Sensitivity contexts are used to reduce the body of a sensitivity abstraction upon application \Trefr{r-inst}, delaying the resource substitution until a value has been reached.
While this is not necessary for a statically-typed language like \SoulCore, it is important for the gradual language \GSoulCore for performing sound runtime checks; we further explain this design decision in \secref{sec:gradual-lang}.}

% We illustrate the dynamic semantics with a simple example. Suppose $e = (\lambda (x:\rtype).x+1) \app 2$, then the reduction sequence is:

% \begin{align*}
%   & (\lambda (x:\rtype).x+1) \app 2\\
%   & \mapsto \lclosure[\emptyvenv]{\lambda (x:\rtype).x+1} \app 2  & \text{\color{black} by \Trefr{r-lam}, \Trefr{R$\rightarrow$} and \Trefr{R$\Ectx$}}\\
%   & \mapsto \ctx(\set{x \mapsto 2}, x + 1)                        & \text{\color{black} by \Trefr{r-app}, \Trefr{R$\rightarrow$}}\\
%   & \mapsto \ctx(\set{x \mapsto 2}, 2 + 1)                        & \text{\color{black} by \Trefr{r-var}, \Trefr{R$\rightarrow$} and \Trefr{Rctx}}\\
%   & \mapsto \ctx(\set{x \mapsto 2}, 3)                            & \text{\color{black} by \Trefr{r-plus}, \Trefr{R$\rightarrow$} and \Trefr{Rctx}}\\
%   & \mapsto 3                                                     & \text{\color{black} by \Trefr{r-ctx}, \Trefr{R$\rightarrow$}}
% \end{align*}

% The reduction steps take care of substituting every instance of $x$, and when the reduction inside a context has reached a final value, the substitution is dropped along with the context, since a value has no free variables.

\paragraph{Properties}
First, \SoulCore is type safe, \ie~every well-typed closed expression is either a value or it can take a step to another expression whose type is a subtype of the original type:

\begin{proposition}[Type safety]
  If $\ssttyping[\emptytenv][\emptysvenv]{e}{\cty}$ then either $e$ is a value $v$, or $\cred[]{e}{e'}$, where $\ssttyping[\emptytenv][\emptysvenv]{e'}{\ctyp}$ and $\ctyp \subty \cty$.
\end{proposition}

Second, sensitivity typing in \SoulCore is sound, \ie~all well-typed expressions satisfy \emph{metric preservation} \cite{reedAl:icfp2010}.
Intuitively, metric preservation states that if a program is s-sensitive, it can only magnify the distance between two inputs by a factor \reviv{of at most} $\sens$.
This property captures the maximum variation of an open expression, if closed with two different substitutions at some arbitrary \emph{distance}, \ie~with respect to an input variation.
For instance, consider
  $e = x + 2y$, typed as
  $\ssttyping[x:\teff{\rtype}{\r}, y:\teff{\rtype}{2\r}][\r]{e}{\teff{\rtype}{5\r}}$.
If we know that the resource $\r$ may vary in at most a magnitude of $2$, \ie~inputs are at \emph{distance} $\SG{2\r}$, then by metric preservation we know that the output will vary at most by $\SG{2\r \cdot 5\r} = 10$, where $\cdot$ corresponds to the dot product of polynomials, \ie~$\SG{(\senv[1] + \sens[1]\r) \cdot (\senv[2] + \sens[2]\r)} = (\senv[1] \cdot \senv[2]) + (\sens[1] * \sens[2])$.
This is the case if we choose two arbitrary \reviv{substitutions} at distance $\SG{2\r}$: $\venv[1] = \set{x \mapsto 2, y \mapsto 4}$ and $\venv[2] = \set{x \mapsto 4, y \mapsto 8}$.\footnote{
  Notice that since $x$ is 1-sensitive in $\r$, two values for $x$ may differ in at most $\SG{2\r \cdot \r} = 2$.
  Similarly, given that $y$ is 2-sensitive in $\r$, two values for $y$ may differ in at most $\SG{2\r \cdot 2\r} = 4$.
  In particular, $\venv[1]$ and $\venv[2]$ satisfy these constraints, thus they are at distance $\SG{2\r}$.
}
\reviv{A substitution $\venv$ is a mapping between variables and values, and we write $\venv(e)$ for an expression where each variable in the domain of $\venv$ has been substituted with its corresponding value.}
Then $\creds[]{\venv[1](e)}{10}$ and $\creds[]{\venv[2](e)}{20}$, and $\abs{10 - 20} \leq 10$, satisfying at runtime the guarantee established statically.
We leave the formal definitions and proofs of these results to the supplementary material. \revii{\S\ref{sec:soundness}} formalizes and explains in detail metric preservation for the gradual language \GSoulCore, which subsumes that of \SoulCore.


==> sections/runtime_semantics.tex <==

\section{Dynamic semantics}
\label{sec:dynamic-semantics}

\begin{revviiib}
In~\S\ref{sec:dynamic-semantics-preview} briefly describe \GSoulEvCore, an enriched version of \GSoulCore, responsible for performing runtime checks during reduction.
We now turn our attention to the details of how this is achieved.
First, in~\S\ref{subsec:evidence}, we describe the mechanism to perform runtime checks and to collect precise runtime information.
Then, in~\S\ref{subsec:intrinsic}, we integrate this mechanism into the syntax of \GSoulEvCore and present its dynamic semantics.
\end{revviiib}

\subsection{Runtime Checks for Gradual Sensitivity}
\label{subsec:evidence}

\begin{revviiib}
In order to perform runtime checks, we follow the approach of~\citet{garciaAl:popl2016}, which uses \emph{evidences} to justify consistent judgments.
Evidences, denoted by the meta-variable $\ev$, are syntactically attached to expressions that rely on consistent judgments, and serve the purpose of \emph{justifying} such judgments.
Furthermore, they can be combined to (try to) justify transitivity of two consistent judgments.
\end{revviiib}
As standard for consistent subtyping, an evidence $\ev$ is represented as a pair of \typeclsPlur, written $\evi{\cgty, \cgty}$, each of which is at least as \emph{precise} as the types involved in the consistent subtyping relation.
\da{revA: \quot{what does each argument of an evidence mean?}}

% Evidence is.
% Then, when trying to justify transitivity of two judgments, their evidences are combined; if the combination is undefined, transitivity is not justified and the program halts with a runtime error.
% Analogous as to having subtyping work for sensitivities, sensitivity effects, \tyclsPlur and \typeclsPlur, evidences can contain a pair of gradual sensitivities, sensitivity effects, \tyclsPlur and \typeclsPlur, respectively.

Evidence is initially computed using the \emph{interior} operator, which essentially produces a refined pair of gradual types from a consistent judgment, based solely on the knowledge that the judgment holds.
Definition \ref{def:interior} shows the interior operator for consistent sensitivity subtyping.
The interior operator for other constructs is inductively defined from the definition for gradual sensitivities and can be found in the supplementary material.

\begin{definition}[Interior]
  \label{def:interior}
  If $\sens[1] \leq \sens[2] \smeet \sens[4]$ and $\sens[1] \sjoin \sens[3] \leq \sens[4]$:
  \begin{align*}
    \Isub(\sensint{\sens[1], \sens[2]}, \sensint{\sens[3], \sens[4]}) =
      \evi{\sensint{\sens[1], \sens[2] \smeet \sens[4]}, \sensint{\sens[1] \sjoin \sens[3], \sens[4]}}
  \end{align*}
  Otherwise, the interior operation is undefined.
\end{definition}

As an example, consider the types $\cgty[1] = \teff{\rtype}{\unknown\r}$ and $\cgty[2] = \teff{\rtype}{10\r}$, noting that $\cgty[1] \ccsub \cgty[2]$.
Then, we can compute the initial evidence for that judgment as $\ev = \Isub(\cgty[1], \cgty[2]) = \evi{\teff{\rtype}{\sensint{0,10}\r}, \teff{\rtype}{\sensint{10,10}\r}}$.
This evidence is said to \textit{justify} the consistent subtyping judgment, written $\ev \evjust \cgty[1] \ccsub \cgty[2]$, which is formally defined as $\ev \gprec^2 \Isub(\cgty[1], \cgty[2])$, where $\gprec^2$ is the precision relation checked component-wise.
\da{revB: \quot{ if we compute $\epsilon = Interior$, does it then make sense to check that $\epsilon \sqsubseteq Interior$? does $\epsilon$ evolve further, if so how?}}

Notice that consistent subtyping is not transitive.
For instance, although $\teff{\rtype}{10\r} \ccsub \teff{\rtype}{\unknown\r}$ and $\teff{\rtype}{\unknown\r} \ccsub \teff{\rtype}{5\r}$, the transitive judgement of both, $\teff{\rtype}{10\r} \ccsub \teff{\rtype}{5\r}$, does not hold.
Therefore, during runtime, evidences need to be \textit{combined} in order to try to justify transitivity of two judgments.
In the case where the combination of two evidences is not defined a runtime error is raised.
Formally, this notion is captured by the \emph{consistent transitivity operator}, denoted $\transsub$.
For instance, suppose $\ev[1] \evjust \teff{\rtype}{\sensval{10}\r} \ccsub \teff{\rtype}{\unknown \r}$ and $\ev[2] \evjust \teff{\rtype}{\unknown \r} \ccsub \teff{\rtype}{\sensval{5}\r}$.
Since $\sensint{10,10}$ is not plausibly smaller than $\sensint{5,5}$ ($10 \nleq 5$), then $\ev[1] \transsub \ev[2]$ should be undefined and an error should be raised.

Definition~\ref{def:ctrans} shows the consistent transitivity operator for sensitivity subtyping.
The consistent transitivity operator for other constructs is inductively defined from the definition for gradual sensitivities and can be found in the supplementary material.

\begin{definition}[Consistent Sensitivity Subtyping Transitivity]
  \label{def:ctrans}
  If  $\sens[11] \leq (\sens[12] \smeet \sens[14] \smeet \sens[22])$ and
      $(\sens[13] \sjoin \sens[21] \sjoin \sens[23]) \leq \sens[24]$:
  \begin{align*}
    &\evi{\sensint{\sens[11], \sens[12]}, \sensint{\sens[13], \sens[14]}} \transsub
    \evi{\sensint{\sens[21], \sens[22]}, \sensint{\sens[23], \sens[24]}} = \\
    &\evi{
      \sensint{\sens[11], \sens[12] \smeet \sens[14] \smeet \sens[22]},
      \sensint{\sens[13] \sjoin \sens[21] \sjoin \sens[23], \sens[24]}
    }
  \end{align*}
  Otherwise, the consistent transitivity operation is undefined.
\end{definition}

Consider again two evidences such that $\ev[1] \evjust \cgty[1] \ccsub \cgty[2]$ and $\ev[2] \evjust \cgty[2] \ccsub \cgty[3]$.
Then, the evidence $\ev[1] \transsub \ev[2]$, if defined, justifies the consistent subtyping judgment $\cgty[1] \ccsub \cgty[3]$, which gives us the ability to perform runtime checks for consistent subtyping.
Next, we come back to the choice using intervals as a mechanism for controlling imprecision.

\paragraph{Sensitivity Intervals in the Runtime Semantics} \label{sec:whyintervals}

Intervals not only provide programmers with a fine-grained mechanism for controlling imprecision; they are also necessary in the design of the runtime semantics \revvi{and for proving metric preservation}.
Fully-precise sensitivities and the unknown sensitivity $\unknown$ fail to retain enough precision to guarantee expected runtime failures, as noted by \citet{toroAl:toplas2018} and their use of security labels intervals in evidence.
\reviv{\citet{banados:arxiv2020} identify this issue as the runtime semantics not enforcing the {\em modular type-based invariants} expected from the static type discipline.}
Let us compare how evidence evolves when we do not use intervals.
\begin{revvib}
We omit the \tyclsPlur for the sake of brevity.
Suppose $\ev[1] \evjust \SG{3\r} \ccsub \SG{5\r}$, $\ev[2] \evjust \SG{5\r} \ccsub \SG{\unknown \r}$ and $\ev[3] \evjust \SG{\unknown\r} \ccsub \SG{4\r}$.
First of all, the interior operator without intervals would yield $\ev[1] = \evi{\SG{3\r}, \SG{5\r}}$, $\ev[2] = \evi{\SG{5\r}, \SG{\unknown \r}}$ and $\ev[3] = \evi{\SG{\unknown\r}, \SG{4\r}}$.
In contrast, with intervals, evidences are computed as $\ev[1] = \evi{\SG{3\r}, \SG{5 \r}}$, $\ev[2] = \evi{\SG{5\r}, \SG{\sensint{5, \infty} \r}}$ and $\ev[3] = \evi{\SG{\sensint{0, 4}\r}, \SG{4\r}}$.
Then if we compute $(\ev[1] \transsub \ev[2]) \transsub \ev[3]$:

% Suppose $\ev[1] = \evi{\SG{\sensval{3}\r}, \SG{\sensval{5}\r}}$, $\ev[2] = \evi{\SG{\sensval{5}\r}, \SG{\unknown \r}}$ and $\ev[3] = \evi{\SG{\sensval{4}\r}, \SG{\sensval{4}\r}}$.
% Let us compute $\ev = (\ev[1] \transsub \ev[2]) \transsub \ev[3]$ with and without using intervals:

\begin{small}
\begin{minipage}{0.15\textwidth}
  \raggedright
  \textit{\black Without intervals:}
\end{minipage}
\begin{minipage}{0.25\textwidth}
  \begin{align*}
    % \ev
    %&= (\ev[1] \transsub \ev[2]) \transsub \ev[3]\\
    &(\evi{\SG{\sensval{3}\r}, \SG{\sensval{5}\r}} \transsub \evi{\SG{\sensval{5}\r}, \SG{\unknown \r}}) \transsub \ev[3]\\
    % &= (\evi{\SG{\sensval{3}\r}, \SG{\unknown \r}}) \transsub \ev[3]\\
    &= \evi{\SG{\sensval{3}\r}, \SG{\unknown \r}} \transsub \evi{\SG{\unknown\r}, \SG{\sensval{4}\r}}\\
    &= \evi{\SG{\sensval{3}\r}, \SG{\sensval{4}\r}}
  \end{align*}
\end{minipage}

\begin{minipage}{0.15\textwidth}
  \raggedright
  \textit{\black With intervals:}
\end{minipage}
\begin{minipage}{0.25\textwidth}
\begin{align*}
  % \ev
  %&= (\ev[1] \transsub \ev[2]) \transsub \ev[3]\\
  & (\evi{\SG{\sensval{3}\r}, \SG{\sensval{5}\r}} \transsub
  \evi{\SG{\sensval{5}\r}, \SG{\sensint{5,\infty} \r}}) \transsub \ev[3]\\
  % &= (\evi{\SG{\sensval{3}\r}, \SG{\sensint{5, \infty} \r}}) \transsub \ev[3]\\
  &= \evi{\SG{\sensval{3}\r}, \SG{\sensint{5, \infty} \r}} \transsub \evi{\SG{\sensint{0,4}\r}, \SG{\sensval{4}\r}}\\
  &~~~\text{which is undefined}\\
\end{align*}
\end{minipage}
\end{small}

In the setting without intervals, the operations do not fail because in the combination of $\ev[1]$ and $\ev[2]$ information is lost.
From the beginning, we can notice that the right-hand side sensitivity of $\ev[2]$ will never be less than $\sensval{5}$.
Nevertheless, the result of the combination, $\evi{\SG{\sensval{3}\r}, \SG{\unknown \r}}$, has no way to encode such information, so later when combined with $\ev[3]$ the operation can not be refuted.
In contrast, the combination using intervals successfully yields an undefined result (since there is no intersection between $\sensint{5, \infty}$ and $\sensval{4}$).
This exemplifies how using only fully-precise sensitivities and the unknown sensitivity $\unknown$ would yield unintended forgetful semantics~\cite{greenberg:popl2015}.

A final key reason as to why use intervals is that they are an expressive enough representation for having associativity of the consistent transitivity operator.
Indeed, with intervals we have that $(\ev[1] \transsub \ev[2]) \transsub \ev[3]$ is equivalent to $\ev[1] \transsub (\ev[2] \transsub \ev[3])$, which is crucial for the soundness proof of \lang.
Furthermore, in the example without intervals, we can observe that associativity is not guaranteed as $\ev[2] \transsub \ev[3]$ is undefined, making the order of the combination of evidences relevant.
\end{revvib}

Equipped with a formal definition of evidences and operations for initially inferring (interior operator) and combining them (consistent transitivity operator), we can now augment the syntax of our gradual language with evidences that can be refined, at runtime, by combining them.
% Recalling the characteristics of gradual languages, evidences serve the purpose of accounting for the optimistic judgments during typechecking.
% Next, we derive the runtime semantics by elaborating \GSoulCore to a language with a richer syntax.


\begin{figure*}[!t]
  \begin{small}
    \begin{align*}
      u ::={}&
        c \mid
        \lambda (x:\gty). e \mid
        \polyS. e
        & \syntaxLabel{simple values} \\
      %
      v ::={}& \ev u \ascr{\cgty}
        & \syntaxLabel{values}\\
      %
      e ::={}&
        v \mid
        \bop \overline{e} \mid
        x \mid
        \ev e \ascr{\cgty} \mid
        e \app e
        \mid
        e \appS{\gsenv} \mid
        \ev \sctx{\r}{\gsenv}(e) \ascr{\cgty}
        & \syntaxLabel{expressions}\\
      E ::={}&
        \emptycontext \mid \bop(\overline{v_i}, \Ectx, \overline{e_j}) \mid \Ectx \app e \mid v \app \Ectx \mid \Ectx \appS{\gsenv} \mid \ev \Ectx \ascr{\cgty} \mid \ev \sctx{\r}{\gsenv}(\Ectx) \ascr{\cgty} & \syntaxLabel{evaluation contexts}
    \end{align*}
  \end{small}

  \textbf{Notions of reduction} \hfill
  \boxed{\ncred{e}{e}}
    \begin{small}


    \begin{align*}
      %
      % PLUS
      %
      \IGrefr{r-op} & &
      \bop \overline{(\ev[i] c_i \ascr{\cgty[i]})}
      &\longrightarrow
      \ev c \ascr{\cgty}\\
      \where & &
      \multicolumn{2}{c}{
      $
        \ev = \bopFuncName^2(\overline{\ev[i]}), \quad
        c = \mathbin{\llbracket \bop\! \rrbracket}\, \overline{c_i}, \quad
        \cgty = \bopFuncName(\overline{\cgty[i]})$
      }\\
      %
      % APP
      %
      \IGrefr{r-app} & &
      (\ev (\lambda (x: \cgtyp[1]).e) \ascr{\cgty}) \app (\ev[1] u \ascr{\cgty[1]})
      &\longrightarrow
      \begin{cases}
        \ev[2]
          ([\evp[1] u \ascr{\cgtyp[1]}/x]e)
         \ascr{\codd(\cgty)} & \\
        \error \hspace{1.7cm} \text{\color{black} if not defined}\\
      \end{cases} \\
      \where &&
      \multicolumn{2}{c}{$
        \cgty[1] = \domm(\cgty), \quad
        \ev[2] = \icod(\ev), \quad
        \evp[1] = \ev[1] \transsub \idom(\ev)
      $}\\
      %
      % APP-SENV
      %
      \IGrefr{r-inst} & &
      (\ev \polyS[\r].e \ascr{\cgty}) \appS{\gsenv}
      & \longrightarrow
      \iinst(\ev, \gsenv)
      \sctx{\r}{\gsenv}(e)
      \ascr{\instt(\cgty, \gsenv)}\\
      %
      % BIG-CTX
      %
      \IGrefr{r-sctx} & &
      \ev \sctx{\r}{\gsenv}(v) \ascr{\cgty}
      & \xlongrightarrow{}
      \ev \substv{\gsenv}{\SG{\r}}{v} \ascr{\cgty}\\
      %
      % ASCR
      %
      \IGrefr{r-ascr} & &
      \ev (\evp u \ascr{\cgtyp}) \ascr{\cgty}
      & \longrightarrow
      \begin{cases}
        (\evp \transsub \ev) u \ascr{\cgty} & \\
        \error & \text{\color{black}if not defined}
      \end{cases}
    \end{align*}
  \end{small}
  \begin{minipage}[t]{0.4\textwidth}
    \textbf{\black Evidence meta-functions}
  \begin{small}
    \begin{align*}
      \idom(\evi{\cgty[1], \cgty[2]}) &= \evi{\domm(\cgty[2]), \domm(\cgty[1])} \\
      \icod(\evi{\cgty[1], \cgty[2]}) &= \evi{\codd(\cgty[1]), \codd(\cgty[2])} \\
      \iinst(\evi{\cgty[1], \cgty[2]}, \gsenv) &= \evi{\instt(\cgty[1], \gsenv), \instt(\cgty[2], \gsenv)} \\
        \bopFuncName^2(\overline{\evi{\cgty[i1], \cgty[i2]}}) &=
          \evi{
            \bopFuncName(\overline{\cgty[i1]}),
            \bopFuncName(\overline{\cgty[i2]})
          }
      \end{align*}
    \end{small}
  \end{minipage}
  \begin{minipage}[t]{0.58\textwidth}

    \textbf{\black Reduction} \hfill
    \boxed{\cred{e}{e}}

    \begin{mathpar}
      \inference[\IGrefr{R$\Ectx$}]{
          e_1
          \longrightarrow
          e_2
      }{
        \cred[]{
          \Ectx[][e_1]
        }{
          \Ectx[][e_2]
        }
      } \and
      \inference[\IGrefr{R$\Ectx$err}]{
        e_1 \longrightarrow \error
      }{
        \cred[]{E[e_1]}{\error}
      }
      % \and
      % \inference[\IGrefr{Rsctx}]{
      %   \cred{t_1}{t_2}
      % }{
      %   \cred[\venv]{
      %     \sctx{\r}{\gsenv}(t_1)
      %   }{
      %     \sctx{\r}{\gsenv}(t_2)
      %   }
      % }
    \end{mathpar}
  \end{minipage}


  \caption{Dynamic semantics of \GSoulEvCore (excerpt)}
  \label{fig:intrinsic-terms-reduction}
\end{figure*}

\subsection{Evidence-based Dynamic Semantics}
\label{subsec:intrinsic}

% \begin{figure}[!t]
%   \begin{small}
%   \begin{minipage}{0.5\textwidth}

%     \begin{align*}
%       u ::={}&
%         c \mid
%         \lambda (x:\gty). t \mid
%         \polyS. t
%         & \syntaxLabel{simple values} \\
%       %
%       v ::={}& \ev u \ascr{\cgty}
%         & \syntaxLabel{values}\\
%       %
%       t ::={}&
%         v \mid
%         \bop \overline{t} \mid
%         x \mid
%         \ev t \ascr{\cgty} \mid
%         t \app t \\
%         \mid {}&
%         t \appS{\gsenv} \mid
%         \ev \sctx{\r}{\gsenv}(t) \ascr{\cgty}
%         & \syntaxLabel{terms}
%     \end{align*}
%   \end{minipage}
%   \begin{minipage}{0.45\textwidth}
%     \textbf{\black Well-typed terms} \hfill
%     \boxed{\ittyping{t}{\cgty}}
%     \begin{mathpar}
%       \inferrule*[lab=\IGrefr{var}]{ }{
%         \ittyping{\iterm{x}{\cgty}}{\cgty}
%       }

%       \inferrule*[lab=\IGrefr{ascr}]{
%         \ittyping{t}{\cgty}\\
%         \ev \evjust \cgty \ccsub \cgtyp
%       }{
%         \ittyping{\ev t \ascr{\cgtyp}}{\cgtyp}
%       }
%     \end{mathpar}
%   \end{minipage}
%   \end{small}

%   \caption{Syntax and Type System of \GSoulEvCore (excerpt)}
%   \label{fig:intrinsic-terms-syntax}
% \end{figure}

As mentioned earlier, the dynamic semantics of \GSoulCore are given by a translation to an internal language, \GSoulEvCore, in which every ascription is accompanied by an evidence that supports the associated consistent subtyping judgment. Concretely, we now have $\ev e \ascr{\cgty}$ instead of simply $e \ascr{\cgty}$.
The typing rules of \GSoulEvCore are defined similarly to \GSoulCore, except that (1) type judgments are enriched with evidence information, (2) values are ascribed simple values, and (3) introduction forms are always ascribed. For instance, the type rule for ascriptions is the following:

\begin{mathpar}
\inferrule*{
  \sttyping{e}{\cgty} \\
  \ev \evjust \cgty \ccsub \cgtyp \\
  \typewfs{\cgtyp}
}{
  \sttyping{\ev e \ascr{\cgtyp}}{\cgtyp}
}
\end{mathpar}

Additionally, and similarly to \cite{toroAl:popl2019}, we heavily rely on a type-directed translation that inserts explicit ascriptions (with their corresponding initial evidences) to: (1) allow reduction rules to preserve the original type of an expression, and (2) simplify the number of necessary reduction rules.
The typing rules of \GSoulEvCore and the type-directed elaboration from \GSoulCore to \GSoulEvCore, written $\itelab{e}{e'}{\cgty}$, are routine and provided in the supplementary material.

Figure \ref{fig:intrinsic-terms-reduction} presents the syntax and notions of reduction for \GSoulEvCore.
The reduction of \GSoulEvCore, denoted $\cred{e}{e'}$, is call-by-value, defined with evaluation contexts.
% Analogous to \GSoulCore, reduction $t \mapsto t'$ denotes that the term $t$ reduces to $t'$.
% An example of the derivation by proof normalization of the reduction rules for \GSoulEvCore can be found in the supplementary material.
Rule \IGrefr{r-op} relies on the meta-definition of $\llbracket \bop\! \rrbracket$ and the evidence is computed using the evidence operator $\bopFuncName^{2}$.
The application rule, \IGrefr{r-app}, uses the inversion functions $\idom$ and $\icod$ in order to compute the new evidences for the body of the closure and to justify optimistic judgments and fail otherwise.
Finally, rule \IGrefr{r-ascr} eliminates ascriptions by keeping only the outer one; consistent transitivity is performed in order to justify the new ascribed (simple) value.
Rule \IGrefr{r-inst} reduces the application of resource abstraction to an $\sctxKW$ context, where the substitution is delayed until the body of the abstraction is reduced, as observable in rule \IGrefr{r-sctx}.

In the rule \IGrefr{r-inst}, if we simply substituted $\r$ by $\gsenv$, we may lose information necessary to refute optimistic static assumptions.
Consider the following example, where $c$ is some constant and the resource $\r[1]$ is in scope: $(\polyS[\r[2]]. c \ascr{\r[1]} \ascr{\unknown\r[1]} \ascr{\r[2]}) \appS{\r[1]}$.
Notice that when comparing effects by consistent subtyping, $\r[1] \ccsub \unknown\r[1]$ and $\unknown\r[1] \ccsub \r[2]$, but $\r[1] \not\ccsub \r[2]$\hide{ (recall that the effect $\r[2]$ is syntactic sugar for $\SG{0}\r[1] + \SG{1}\r[2]$)}.
Although, this program typechecks statically, it should fail at runtime, since clearly $\SG{1\r[1]}$ is not a sub-effect of $\SG{1\r[2]}$.
However, if we immediately substitute $\r[2]$ by its instantiation, $\r[1]$, we would get $x \ascr{\unknown\r[1]} \ascr{\r[1]}$, which is going to silently reduce without errors, exposing an inconsistency between the type invariants in the static and dynamic semantics.
In order to avoid this problem, we delay the substitution using a $\sctxKW$ context to first reduce the body of the abstraction and then perform the substitution. %
%
%\footnote{A similar issue also arises in the context of gradual {\em parametricity}~\cite{toroAl:popl2019,ahmedAl:icfp2017}. A stereotypical example is the expression $(\Lambda X. 1 :: \? :: X) [ \mathsf{Int} ]$, which ought to fail, despite the coincidental match between the type of the literal $1$ and the instantiated type for $X$. Notice how: (1) the expression optimistically typechecks, as both $\mathsf{Int} \sim \?$ and $\? \sim X$ hold; and (2) a runtime error should be expected, as $\mathsf{Int} \not\sim X$.
%Gradually-parametric languages usually tackle this issue by adopting {\em runtime sealing}, \ie~a type application reduces using a sealing substitution with a fresh global type name~\cite{matthewsAhmed:esop2008}.}
This way, evidences preserve the information necessary to refute optimistic judgments when trying to justify transitivity in rule \IGrefr{r-ascr}. Finally, reduction rules \IGrefr{R$\Ectx$} and \IGrefr{R$\Ectx$err} reduce subexpressions  within evaluation contexts and propagate errors, respectively.
The example term therefore reduces as follows:
% to $\sctx{\r[2]}{\r[1]}(c \ascr{\r[1]} \ascr{\unknown\r[1]} \ascr{\r[2]})$ which will error, since the transitivity of the ascriptions will fail before the substitution is performed.

%\et{the reduction arrow is not defined -- is this short version the same as the one used in the following section?}

\begin{small}
  \begin{align*}
    (\polyS[\r[2]]. c \ascr{\r[1]} \ascr{\unknown\r[1]} \ascr{\r[2]}) \appS{\r[1]}
    &\underbrace{\cred[]{}{}}_{\text{..., \IGrefr{r-inst}}}
    \sctx{\r[2]}{\r[1]}(c \ascr{\r[1]} \ascr{\unknown\r[1]} \ascr{\r[2]}) \\
    &\underbrace{\cred[]{}{}}_{\text{..., \IGrefr{r-ascr}}}
    \cred[]{\sctx{\r[2]}{\r[1]}(\error)}{\error}
  \end{align*}
\end{small}

\begin{comment}

\paragraph{Elaboration} \label{subsec:gradual:dynamics:elaboration}
So far, we have defined the runtime semantics of \GSoulEvCore that, by translation, also defines the runtime semantics for \GSoulCore.
% We now formalize the elaboration of terms from \GSoulCore to \GSoulEvCore and establish that it preserves typeability.
% Figure \ref{fig:intrinsic-elaboration} illustrates the elaboration from gradual expressions to evidence-augmented intrinsic terms.
Judgment $\itelab{e}{t^{\cgty}}{\cgty}$ denotes the elaboration of the intrinsic term $t^{G}$ from the expression $e$, where $e$ has type $\cgty$ under the type environment $\tenv$ and a resource set $\svenv$.
The rules of elaboration simply perform the transformations mentioned at the beginning of this section and are presented in the supplementary material.
However, as an example, we present the rule for elaborating ascribed expressions, which showcases the use of the interior operator to produce the initial evidence to justify the ascription:

\begin{small}
\begin{align*}
  \inferrule*[lab=\ELrefr{ascr}]{
    \itelab{e}{t}{\cgty}\\
    \typewfs{\cgtyp}\\
    \ev = \Isub(\cgty,\cgtyp)
  }{
    \itelab{e \ascr{\cgtyp}}{
      \ev t \ascr{\cgtyp}
    }{\cgtyp}
  }
\end{align*}
\end{small}

% \begin{figure}[!tp]
%   \begin{small}

%   \textbf{Elaboration of Intrinsic Terms} \hfill
%   \boxed{\itelab{e}{t^{\cgty}}{\cgty}}\\

%   \begin{mathpar}
%   \inferrule*[lab=\ELrefr{const}]{
%     \ev = \Isub(\constty(c),\constty(c))
%   }{
%     \itelab{c}{\ev c \ascr{\constty(c)}}{\constty(c)}
%   }

%   \inferrule*[lab=\ELrefr{ascr}]{
%     \itelab{e}{t}{\cgty}\\
%     \typewfs{\cgtyp}\\
%     \ev = \Isub(\cgty,\cgtyp)
%   }{
%     \itelab{e \ascr{\cgtyp}}{
%       \ev t \ascr{\cgtyp}
%     }{\cgtyp}
%   }

%   \inferrule*[lab=\ELrefr{app}]{
%     \itelab{e_1}{
%       t_1
%     }{\cgty[1]}\\
%     \itelab{e_2}{t_2}{\cgty[2]}\\
%     \ev[2] = \Isub(\cgty[2], \domm(\cgty[1]))
%   }{
%     \itelab{
%       e_1 \app e_2
%     }{
%       t_1 \app
%       (\ev[2] t_2 \ascr{\domm(\cgty[1])})
%     }{\codd(\cgty[1])}
%   }
%   \end{mathpar}
%   \end{small}

%   \caption{Elaboration from  \GSoulCore to \GSoulEvCore  (excerpt)}
%   \label{fig:intrinsic-elaboration}
% \end{figure}

% Rules \ELrefr{const} and the ones for elaborating functions insert ascriptions and justify them with evidences produced by the interior operator.
% The computation of these evidences never fails since both \typeclsPlur{} are always the same, so the insertion of these ascriptions \revii{is} harmless.
% Rule \ELrefr{app} ascribes the argument by the expected \tyclsSing{} while preserving its sensitivity effect.
% The interior operator is used again to produce the evidence with the difference that this computation may fail if $\cgty[2]$ is not a subtype of $\domm(\cgty[1])$.
% Finally, \ELrefr{ascr} produces an initial evidence to justify the ascription.
% This ascription can also fail to compute if subtyping is not satisfied.

% In order to conclude with the derivation of the dynamic semantics of \GSoulEvCore we establish that elaboration preserves typing.
Finally, we note that, after typing, elaboration rules only insert trivial ascriptions and enrich derivations with evidence and ascriptions.
As this derivations are represented as intrinsic terms, by construction, elaboration of terms trivially preserves typing.

\begin{proposition}[Elaboration preserves typing]
  \label{prop:elab-preserves-typing}
  If $\sttyping{e}{\cgty}$, then $\itelab{e}{t}{\cgty}$ and $\ittyping{t}{\cgty}$.
\end{proposition}

% \paragraph{A Note on Following the AGT Framework}
% \AGT{
% Even though \GSoulCore is systematically derived using AGT, the application of this framework to sensitivity typing in \SoulCore presents a number of challenges valuable to readers already familiar with the methodology: the possibly-bounded treatment of imprecision, consistent sensitivity subtyping , \reviv{a sound representation for evidence, and the derivation of the runtime semantics}.
% Finally, AGT provides no guidance whatsoever for preserving soundness of typing for hyperproperties like gradual metric preservation, which is one of the main technical contributions of this work.
% For more technical details on the application of AGT to sensitivity typing, we refer the reader to the supplementary material.
% }
\end{comment}

